Locate-then-edit for Multi-hop Factual Recall under Knowledge Editing

The locate-then-edit paradigm has shown significant promise for knowledge editing (KE) in Large Language Models (LLMs). While previous methods perform well on single-hop fact recall tasks, they consistently struggle with multi-hop factual recall tasks involving newly edited knowledge. In this paper, leveraging tools in mechanistic interpretability, we first identify that in multi-hop tasks, LLMs tend to retrieve knowledge with implicit subject information from deeper MLP layers, unlike single-hop tasks, which rely on shallow layers. This distinction explains the poor performance of current methods in multi-hop queries, as they primarily focus on editing shallow layers with single-hop edit prompts, leaving deeper layers unchanged. To address this, we propose IFMET, a novel locate-then-edit KE approach designed to edit both shallow and deep MLP layers. Beyond single-hop editing prompts, IFMET further incorporates multi-hop editing prompts to locate and modify knowledge across different stages of reasoning. Experimental results demonstrate that IFMET significantly improves performance on multi-hop factual recall tasks, overcoming the limitations of previous locate-then-edit methods

==> ICLR_Version/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR_text/abstract.tex <==
\begin{abstract}
The locate-then-edit paradigm has shown significant promise for knowledge editing (KE) in Large Language Models (LLMs). While previous methods perform well on single-hop fact recall tasks, they consistently struggle with multi-hop factual recall tasks involving newly edited knowledge. In this paper, leveraging tools in mechanistic interpretability, we first identify that in multi-hop tasks, LLMs tend to retrieve implicit subject knowledge from deeper MLP layers, unlike single-hop tasks, which rely on earlier layers. This distinction explains the poor performance of current methods in multi-hop queries, as they primarily focus on editing shallow layers, leaving deeper layers unchanged. To address this, we propose IFMET, a novel locate-then-edit KE approach designed to edit both shallow and deep MLP layers. IFMET employs multi-hop editing prompts and supplementary sets to locate and modify knowledge across different reasoning stages. Experimental results demonstrate that IFMET significantly improves performance on multi-hop factual recall tasks, effectively overcoming the limitations of previous locate-then-edit methods.


%As the need to update their knowledge grows, effective knowledge editing (KE) methods are crucial for Large Language Models . Current approaches, such as the locate-then-edit paradigm, modify internal model weights but struggle with multi-hop factual recall tasks, where edited knowledge fails to propagate to deeper layers of reasoning.

%Existing knowledge editing techniques modify a minor proportion of knowledge in Large Language Models (LLMs) to address issues of outdated and incorrect information. While these methods have shown notable success for single-hop queries, they exhibit limitations when applied to multi-hop fact recall tasks, particularly those involving weight-modifying techniques known as locate-then-edit. Our investigation into the poor performance of these locate-then-edit methods attributed their failures to incomplete knowledge updates, especially in the later MLP layers. In response, we proposed a new method, \underline{\textbf{I}}nterpretability-Guided \underline{\textbf{F}}urtherance \underline{\textbf{M}}odel \underline{\textbf{E}}diting in a \underline{\textbf{T}}ransformer \textbf{(IFMET)}. By integrating a supplementary set comprised of multi-hop edit prompts into exiting knowledge editing methods and conducting a furtherance edit, IFMET achieves a comprehensive update of the model's internal knowledge. We validated the effectiveness of IFMET using the GPT-J model on the MQuAKE dataset, demonstrating its superior performance in handling complex multi-hop fact recall tasks.

\end{abstract}

==> ICLR_text/algorithm/IFMET.tex <==
\setlength{\algomargin}{10pt}
\RestyleAlgo{ruled}
\newlength{\commentWidth}
\setlength{\commentWidth}{7cm}
\newcommand{\atcp}[1]{\tcp*[f]{\makebox[\commentWidth]{#1\hfill}}}
\newcommand{\atcpl}[1]{\tcp*[r]{\makebox[\commentWidth]{#1\hfill}}}
\newcommand\mycommfont[1]{\footnotesize\textcolor{blue}{#1}}
\newcommand{\elid}[2]{#1_{#2}}
\newcommand{\tresid}{\elid{\delta}{i}}
\newcommand{\prsub}[2]{\mathbb{P}_{#2}\left[ #1 \right]}
\newcommand{\atl}[2]{#1^{#2}}
\newcommand{\refeqn}[1]{Eqn.~\ref{eq:#1}}
\newcommand{\method}{MEMIT\xspace}
\newcommand{\Gsub}{G(\atl{h}{L}_i\mathrel{+}=\tresid)}
\SetCommentSty{mycommfont}
\begin{center}
\scalebox{0.9}{
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
\SetAlgoLined
\caption{IFMET}\label{alg:mrome}
\KwData{Requested edits $E = \{ (s_i, r_i, o_i\to o_i^*) \}_{i=1}^N$, Supplementary set $Sup={\{(s'_i,r'_i,s_i)\}_{i=1}^N}$, model $\mathcal{M}$ , first edit layers $l_1$, furtherance edit layers $l_2$}
\KwResult{Modified model $\mathcal{M}_{E}$ containing edits from $E$}

\For (\quad \atcp{First Edit Process}){$(s_i, r_i, o^*_i)\in E$}{
    \textbf{Generate the single edit prompt} $T_{r_i}(s_i)$ \;
    \textbf{Optimize} $v^*_i \gets Search(T_{r_i}(s_i)$)  \atcpl{$v^*_i$ for every new fact}
}
\For(\quad \atcp{Update weights of Shallow MLPs}){$l \in l_1$}{
    $\Delta^l \gets Calculate([v^*_1,\dots,v^*_N]) $  \quad \atcpl{Compute weight change with target vectors}
    $W^l \gets W^l + \Delta^l$ \quad \atcpl{Update layer $l$ MLP weights in model}
}
\For (\quad \atcp{Furtherance Edit Process}){$(s'_i,r'_i,s_i) \in Sup$}{
    \textbf{Construct the multi-hop Chain} $C = (s'_i,r'_i,s_i)\oplus(s_i,r_i,o)$ \;
    \textbf{Generate the multi-hop edit prompt} $T_C(s'_i)$ \;
    \textbf{Optimize} $v^*_i \gets Search(T_{C}(s'_i)$) \;
}
\For(\quad \atcp{Update weights of Deeper MLPs}){$l \in l_2$}{
    $\Delta^l \gets Calculate([v^*_1,\dots,v^*_N]) $  \;
    $W^l \gets W^l + \Delta^l$
}
\end{algorithm}%
\end{minipage}%
}%
\end{center}


==> ICLR_text/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}
\vspace{-0.1in}
We focused on developing locate-then-edit knowledge editing methods for multi-hop factual recall tasks. 
We first verified that in multi-hop tasks, LLMs tend to retrieve implicit subject knowledge from deeper MLP layers, unlike single-hop tasks, which rely on earlier layers. This distinction explains the poor performance of current methods in multi-hop queries, as they primarily focus on editing shallow layers, leaving deeper layers unchanged. We then proposed IFMET, a novel locate-then-edit KE approach designed to edit both shallow and deep MLP layers.  Experimental results demonstrate that IFMET significantly improves performance on multi-hop factual recall tasks.


==> ICLR_text/edit_impact.tex <==
\definecolor{rred}{rgb}{0.75, 0.0, 0.0}
\definecolor{bblue}{rgb}{0.13, 0.67, 0.8}

\newcommand{\badmetric}[1]{{\color{rred} \textbf{#1}}}
\newcommand{\goodmetric}[1]{{\color{ggreen} \textbf{#1}}}
\definecolor{ggreen}{rgb}{0.0, 0.6, 0.0}


\subsection{Why Existing locate-then-edit KE Methods Failed}

\addtolength{\tabcolsep}{-3pt}
\begin{wraptable}{R}{0.50\textwidth}
    \centering
    \caption{\small Comparison of QA and Cloze Formats for $D_{Pre}$ and $D_{Post}$}
    \label{tab:prepost-results}
    \scriptsize
    \begin{adjustbox}{width=0.5\textwidth}
    \centering
        \renewcommand{\arraystretch}{1.5} % 设置行间距
        \begin{tabular}{
            l % 左对齐文本
            S[table-format=2.2] S[table-format=2.2] % 对齐两列数值用于QA Format (Pre, Post)
            S[table-format=2.2] S[table-format=2.2] % 对齐两列数值用于Cloze Format (Pre, Post)
            }
        \toprule
        \textbf{Edit Batch} & \multicolumn{2}{c}{\textbf{QA Format(\%)}} $\uparrow$ & \multicolumn{2}{c}{\textbf{Cloze Format(\%)}} $\uparrow$ \\
         & {$D_{Pre}$} & {$D_{Post}$} & {$D_{Pre}$} & {$D_{Post}$} \\
        \midrule
        GPT-J    & 50.62 & 41.72  & 20.31  & 18.63  \\
        \midrule
        Edit=1   & \goodmetric{64.29}  &  \badmetric{2.93} &  \goodmetric{43.37} & 4.60  \\
        Edit=100 & 63.27 & 3.35 & 42.86 & \badmetric{3.35}  \\
        \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{wraptable}
\addtolength{\tabcolsep}{3pt}
Based on the findings above, we can provide an explanation for the unsatisfactory performance of the existing locate-then-edit methods. For an editing instance \( (s, r, o \to o^*) \), using only the corresponding explicit single-hop prompt for editing is insufficient as previous methods only update the relevant knowledge in the shallow MLP layers but fail to propagate the changes to deeper layers, which is utilized in multi-hop fact recall tasks. 

We provide a concrete example for a better understanding. Given an editing instance \( (Spain, captical, Madrid \to Hartford) \), and $Q_{cloze}(s)$ is ``The capital city of Spain is". Existing methods modify the weights of shallow MLPs with $Q_{cloze}(s)$ to make it answer \textit{Hartford}. The paradigm may be well-suited for cases where the modified information is queried in a single-hop manner, as these tasks retrieve answers from the early MLP layers. However, it will be ineffective when the modified knowledge is queried in the second or later fact recall steps, where the model relies on deeper MLP layers at the last token position for knowledge retrieval. In this example, the first-hop query ``The capital city of Spain is located in the continent of" should be answered correctly because it retrieves the knowledge \( (Spain, captical,  Hartford) \) in shallow MLPs. However, the second one ``The capital city of the country has nationals Pablo Picasso is" is still answered with \textit{Madrid} because the knowledge \( (Spain, captical, Madrid) \) stored in later MLPs does not changed.

To verify our above claim, we divide two-hop fact recall tasks into two sets  $D_{Pre}$ and $D_{Post}$, depending on the position of the edited knowledge within the two-hop reasoning process. Specifically, for an edited  knowledge $\left( s, r, o , o* \right)$,  we have the following two sets after editing.
\begin{align*}
D_{Pre} = \{\left( s, r, o^* \right) \oplus \left( s_2, r_2, o_2 \right)\}, \quad D_{Post} = \{\left( s_1, r_1, o_1 \right) \oplus \left( s, r, o^* \right)\}.
\end{align*}
We sampled two subsets with approximately equal size from the MQuAKE-CF dataset, detailed in the Appendix ~\ref{a:pre-post}. By applying the SOTA locate-then-edit method PMET to layer [3-8], which follows~\citep{pmet}, we present the percentage of cases where both pre-edited and post-edited models answer successfully in QA format or Cloze format under different edit batches. 

Table \ref{tab:prepost-results} shows the results of the comparative experiments. We can see that performance on $D_{Pre}$  is significantly better than on $D_{Post}$, which aligns with our expectations. This is because reasoning the first hop knowledge in $D_{Pre}$ is similar to the single-hop process. After updating the knowledge in the earlier MLP layers, the model is likely to effectively use the newly edited knowledge. It can use the new implicit subject in the second hop to produce the final updated answer.  When facing cases in $D_{post}$, PMET cannot get the correct final answer because it only modifies the earlier MLP layers, which is not enough for the model to correctly reason the second hop knowledge as it should be retrieved from later MLP layers. 

%However, when the post case in $D_{Pre}$ resolved the implicit subject and wants to utilize it to retrieve the new answer, there is no updated knowledge in later MLPs to be used. 

\iffalse 
\begin{tcolorbox}[mydefinition={Finding 4}]
Existing methods fail to solve multi-hop problems, especially when the edited fact is utilized in implicit fact recall steps, \textbf{due to their inability to modify knowledge in the deeper MLP layers}.
\end{tcolorbox}
\fi 

==> ICLR_text/experiments.tex <==
\vspace{-15pt}
\section{Experiments}
\vspace{-10pt}
\subsection{Experimental Setup}

\noindent {\bf Dataset.} We use MQuAKE-3K~\citep{MQUAKE}, a challenging dataset designed to evaluate models' ability to perform multi-hop reasoning with newly edited knowledge. Each entry consists of multiple single-hop edits and includes multi-hop reasoning questions.

\noindent {\bf Baselines.} As \textbf{IFMET} is a locate-then-edit approach, we mainly compare it with previous weight-modifying approaches. Specifically, 
our baseline includes the following methods: \rebuttal{\textbf{Base}, which refers to the original model without any edits}; \textbf{ROME}~\cite{ROME}, which identifies editing areas using causal mediation analysis framed as a least-squares problem under linear equality constraints and solving it using Lagrange multipliers; \textbf{MEND}~\cite{MEND}, which employs meta-learning to train a hypernetwork for inferring weight updates from gradients; \textbf{MEMIT}~\cite{MEMIT}, which extends ROME to edit a large set of facts by updating weights in a range of layers; \textbf{MeLLo}, which manages multi-hop knowledge editing by decomposing subproblems and detecting conflicts; \textbf{PMET}, which optimizes FFN hidden states for precise weight updates, achieving SOTA performance in COUNTERFACT~\citep{ROME} and ZsRE~\citep{zsre}.

\noindent {\bf Setup and Hyperparameters.} \rebuttal{To evaluate the performance of different KE methods, we adopt Multi-hop question answering accuracy(Multi-hop Acc) as the primary metric. For each query, the \textbf{unedited answer} denotes the expected old fact before knowledge editing, while the \textbf{edited answer} represents the expected new fact after editing. Unless otherwise specified, we report the performance of \textbf{Base} in generating the \textbf{unedited answer} to reflect the original ability of model to leverage knowledge. For the edited model, we report its accuracy in producing the \textbf{edited answer}, thereby assessing the effectiveness of the editing method. Our experiments are mainly conducted on the GPT-J (6B) model.} We use \text{PMET} as our primary experimental method for both the first and furtherance edits and construct a supplementary set from the knowledge triples of MQuAKE-3K to support our \textbf{IFMET}. Additional details are presented in Appendix~\ref{experiment-setting}. 

\input{text/results/main_result}
\subsection{Experimental Results}
\noindent {\bf General performance.} Table~\ref{tab:main_result} demonstrates the performance of various established methods alongside \textbf{IFMET}  on MQuAKE-3K. We can easily see the previous weight-modifying approaches generally exhibited poor performance. As the edit batch size increases, all methods except PMET show a certain downward trend. Our method inherits the good batch editing ability of PMET and consistently outperforms all others, showcasing a leading edge. Our approach significantly improves upon existing knowledge editing techniques, demonstrating the effectiveness and necessity of updating knowledge storage in deeper MLP layers. \rebuttal{Additionally, we conducted comprehensive ablation study and discussions on generalizability. For detailed results and analyses, please refer to Appendix~\ref{a:ablation_study}}.

\noindent {\bf Effect of number of hops.} Table~\ref{tab:hop_result} in the Appendix displays the performance trends of various knowledge editing methods with different numbers of hops in multi-hop factual recall. We can see that each additional reason hop will negatively impact performance. Notably, IFMET  is the best one in all cases, with minimal performance degradation. In particular, its results are close to those of the original model in the two-hop scenarios. This slight decrease underlines IFMET's robustness and its superior ability to handle complex multi-hop tasks effectively.

\noindent {\bf Effect of the number of edited instances.} We then consider the performance with different edited instances, which refer to the required number of new knowledge updates in the edit case. The results shown in Appendix Table~\ref{tab:edit_result} indicate a performance decline across all methods as more edits are introduced. Notably, IFMET  consistently outperforms other approaches, showing the smallest average decline across different instance scenarios.  Surprisingly, IFMET achieves an accuracy distribution that is close to that of the original model. It is also the only method that maintains excellent performance in complex two-hop and four-hop scenarios, which even outperforms single-hop cases. This can be more visually observed in Appendix Figure~\ref{fig:comparison_of_methods}. 

\noindent {\bf Effect of the edit position.}  As previously mentioned, the same single-hop fact requires different layers to provide knowledge, depending on its position in the multi-hop reasoning chain, involving the earlier and later MLPs. By categorizing according to position, we can assess whether the editing methods have comprehensively updated the relevant knowledge in the model rather than just making partial updates. We classify the edited case according to its position in the relevant multi-hop reasoning chain as Pre, Mid, and Post. For instance, in a three-hop knowledge sequence, editing the first hop is classified as pre, the second as mid, and the third as post. Please refer to  Appendix~\ref{a:editing-position} for the classification of more complex, multi-edit scenarios. To assess the completeness of our method, we evaluated its performance for both eliminating original knowledge and incorporating new knowledge. As detailed in Table~\ref{tab:position_result}, our method significantly enhances outcomes across all classification types—Pre, Mid, and Post. Notably, it achieves exceptional improvements in both modifying new knowledge and eliminating original knowledge, especially in cases classified as Post.
\input{text/results/original_result}

==> ICLR_text/exploration.tex <==
\definecolor{logits-final-a}{HTML}{23A3C2}
\definecolor{logits-inter-a}{HTML}{FF9300}


\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{./pdf/2-hop_logitlens.pdf}
        \caption{Two-hop}
        \label{fig:two-hop-logitlens}
    \end{subfigure}
        % \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{./pdf/1-hop_logitlens.pdf}
        \caption{Single-hop}
        \label{fig:one-hop-logitlens}
    \end{subfigure}
    \caption{\textbf{LogitLens results of the last token position at different layers. } (a) \textcolor{logits-inter-a}{Yellow line} represents the information containing  implicit subject $s_2$, i.e., $\text{Info}(h_l,s_2)$. \textcolor{logits-final-a}{Blue line} represents the information for the final answer, i.e.,  $\text{Info}(h_l,o_2)$.  (b) \textcolor{logits-inter-a}{Yellow line} represents the information of subject $s$. i.e., $\text{Info}(h_l,s)$ and \textcolor{logits-final-a}{Blue line} represents the information of the answer $o$, i.e., $\text{Info}(h_l,o)$. Larger versions of the sub-figures are available in the Appendix~\ref{fig:larger_one-hop-logitlens}.} 
\end{figure}

 \vspace{-0.25in}
\section{Mechanisms of Knowledge Storage and Reasoning}
\label{sec:Mechanisms of Knowledge Storage and Reasoning}
In this section, we will explore the reasoning mechanisms of the pre-edited model for both single-hop and multi-hop factual recall tasks. By comparing the knowledge utilization processes, we identify the reasons behind the suboptimal performance in multi-hop tasks and explain why the post-edited model tends to output the original answer instead of the new edited one. Specifically, we focus on two-hop tasks to better illustrate these distinctions. Experiments are conducted using a subset of single and two-hop data from MQuAKE-CF \citep{MQUAKE} with the GPT-J (6B) model \citep{GPT-J}. More detailed information about the data and experimental setup is provided in Appendix~\ref{a:why-subset}.


\subsection{How the Pre-edited Model Reasons Fact Recall Tasks}
For a multi-hop fact recall task, the knowledge chain is represented as \(C = \left( s_1, r_1, o_1 \right) \oplus \dots \oplus \left( s_n, r_n, o_n \right)\). The model may employ multiple strategies to answer such tasks, including the formation of a single super-relation~\citep{shortcuts} \( (s_1, r_{mul}, o_n) \), where \( r_{mul} = r_1 \to \dots \to r_n \), or by segmenting the task into one explicit recall step followed by several implicit recall steps to answer step-by-step. Previous research~\citep{hou-comp-reason} suggests that models typically engage in reasoning by considering each single-hop recall individually.

Based on this understanding, we hypothesize that the model will prioritize deducing the implicit subjects \(\{s_2, \dots, s_{n}\}\) and subsequently recall the final answer \(o_n\) based on the last implicit subject \(s_n\). The subsequent sections aim to verify this hypothesis by examining the model's behavior in structured multi-hop fact recall tasks.

\noindent {\bf Interpretation via Hidden Representations.}
We use LogitLens to examine the accumulation of information related to the implicit subject \(s_2\) and the final answer \(o_2\) in the two-hop scenario. The model's predictions for \(o_2\), are derived from the last token of the prompt, where crucial information about the resolved implicit subject \(s_2\) should be propagated~\citep{hoptoolate}. Therefore, we focus on the hidden state \(h_l\) at the \(l\)-th layer of the last token position, analyzing \( \text{Info}(h_l, s_2) \) and \( \text{Info}(h_l, o_2) \) as measures of the information related to \(s_2\) and \(o_2\) contained in \(h_l\). Intuitively, these metrics quantify how much information about \(s_2\) and \(o_2\) accumulates in the hidden state. The results, depicted in Figure~\ref{fig:two-hop-logitlens}, show that \( \text{Info}(h_l, s_2) \) gradually reaches its peak during middle layers [15-17], while \( \text{Info}(h_l, o_2) \) increases and peaks during later layers [21-23]. This pattern suggests that, in multi-hop tasks, the implicit subject \(s_2\) is processed during the middle layers before reaching the final answer \(o_2\).

To explore if single-hop fact recalls \((s, r, o)\) follow the same trend as in multi-hop cases, we conducted a similar experiment using LogitLens. The results, shown in Figure~\ref{fig:one-hop-logitlens}, indicate that \( \text{Info}(h_l, s) \) significantly increases after layer 24 and peaks at layer 27, whereas \( \text{Info}(h_l, o) \) consistently reaches its peak during layers 21,22,23. This finding implies that there is no significant peak for the subject information before the final answer probability begins to accumulate, suggesting that the accumulation process of the final answer in single-hop cases may not be significantly correlated with the subject information at the last token.

\begin{tcolorbox}[mydefinition={Takeaway 1}]
In multi-hop scenarios, the implicit subject information consistently accumulates before the final answer at the last token position. However, in single-hop scenarios, since the subject is explicitly given, there is no need for accumulation at the last token position.
\end{tcolorbox}
\vspace{-0.2in}
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{./pdf/2-hop_causal.pdf}
        \caption{Causal intervention results of layer hidden state in last token position.}
        \label{fig:causal_intervent_layer}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{./pdf/mlp_intervent.pdf}
        \caption{Causal Intervention result of MLP hidden state in last token position}
        \label{fig:causal_intervent_mlp}
    \end{subfigure}
\caption{\textbf{Causal Intervention Result}: A brighter color signifies a stronger intervention effect. In each subfigure, upper row represents experimental group, while upper row is control group. Note that negative effect values ($\leq$ 0) are clipped to 0 in both groups for better visualization. (a) is probability change $IE_h$ of intervention $\mathcal{I}_h$, (b) is probability change $IE_m$ of intervention $\mathcal{I}_m$.}
    \label{fig:causal_intervent}
\end{figure}


\noindent {\bf Causal Intervention.} 
Next, we explore whether the appearance of \(s_2\) guides the subsequent information accumulation process of the final answer \(o_2\). To this end, we aim to identify which layers facilitate this influence. We propose an intervention experiment where we reduce the information content of \(s_2\) at the last token position and observe the changes in the output probability of the final answer in the last prediction layer. 

Specifically, we replace the hidden state \(h_l\) in layer \(\ell\) of the last token with \(h^*_l\), and the corresponding logits \(s_l\) (\(= W_U h_l\)) and \(s^*_l\) (\(= W_U h^*_l\)) for \(h_l\) and \(h^*_l\), respectively. \(s^*_l\) is defined as:
\begin{equation}\label{eq:logitsinter}
s^*_l[j] = 
\begin{cases}
    \min(s_l[j]), & \text{if } j \in s_2 \\
    s_l[j], & \text{otherwise},
\end{cases}
\end{equation}
where we minimize the logits corresponding to the tokens in \(s_2\) without altering the values of other tokens, aiming to diminish the effect of \(s_2\). This setup allows us to describe the process through a causal intervention framework, where the intervention \(\mathcal{I}_h\) and the effect \(IE_h\) are defined as follows:
\begin{align}\label{eq:causal}
\mathcal{I}_h : h^*_l = h_l + \argmin_{\Delta h_l} \| W_U(h_l+\Delta h_l) - s^*_l \|^2 ,\quad IE_h = p_L[j] - p_L^E[j], \quad j \in o_2,
\end{align}
where \(L\) is the last layer, \(p_L[j]\) denotes the original output probability of \(o_2\) in the \(L\)-th layer, and \(p^E_L[j]\) is the probability after the intervention is applied. This approach illustrates how the hidden states and probabilities are expected to change when the logits are modified to \(s^*\). For computational efficiency, we opt to approximate \(h^*_l\) using a combination of least squares and minimum-norm methods~\citep{minimum-norm} (further details are provided in Appendix~\ref{a:minimum-norm}).

For comparison,  we also randomly select an irrelevant token $j \notin s_2 \cup o_2$ to execute the intervention as the control group. 
Figure \ref{fig:causal_intervent_layer} presents the outcomes of our intervention experiments across all layers, where a brighter color signifies a stronger intervention effect. 
We found a clear positive impact from intervening in layers [17-19] for the experimental group, in contrast to no significant effects observed in the control group across all layers. This suggests that the information of $s_2$  encoded in the intermediate layers plays a crucial role in the probability accumulation process of $o_2$. We also do the same causal intervention experiments for single-hop fact recall (see Appendix ~\ref{a:causal_1_hop} for the results). However, the results indicate that the prediction of $o$ does not significantly rely on the subject information $s$ in the single-hop fact recall. 
\begin{tcolorbox}[mydefinition={Takeaway 2}]
Unlike the mechanism of reasoning the knowledge in single-hop scenarios, in the reasoning process of the second-hop knowledge in two-hop scenarios, the accumulated subject information has causal effects on the final answer, guiding the extraction of related knowledge in the last layer. 
%During implicit recall steps in multi-hop, \textbf{the accumulation of implicit subject information at the last token position has a causal effect on improving the probability of the final answer}, guides the extraction of related knowledge in the layer layers.
\end{tcolorbox}




\noindent {\bf Intermediate Reasoning Results Influence the Knowledge Extraction from MLP.}
As previous studies claimed that single-hop tasks retrieve subject information from MLP layers~\citep{ROME,meng2022mass}, we will focus on MLP layers to further investigate the specific mechanisms to answer how the implicit subject $s_2$ influences the prediction of the final answer $o_2$.
We conducted a causal intervention experiment similar to the experiments above but focused specifically on the MLP component. Specifically, we aim to replace \(m_l\) (the output hidden state of the last token in the $l$-th MLP layer) with \( m^*_l \),  where we have \( s_l = W_U m_l \) and \( s^*_l = W_U m^*_l \) with $s^*_l$ is same as in~(\ref{eq:logitsinter}). The 
intervention $\mathcal{I}_m$ shares the same idea as in~(\ref{eq:causal}), except that \(h_l\) is replaced with \(m_l\). However, we redefine the intervention effect $IE_m$, which differs from the previous $IE_h$. In detail, we no longer use the probability at the final layer as the metric; instead, we use the probability calculated from the output of MLP at the modified layer $l$. 
In total, our causal intervention is formulated as  
\begin{align*}
\mathcal{I}_m : m^*_l = m_l + \argmin_{\Delta m_l}  \| W_U(m_l+\Delta m_l) - s^*_l \|^2,\quad IE_m =  p_l[j] - p_l^E[j], \quad j\in o_2.
\end{align*}
Figure \ref{fig:causal_intervent_mlp} presents the outcomes of our intervention experiments across all layers with the similar control group as in the above.\footnote{Note that, considering the tiny output probability of MLP, we did not use normalization of probability changes here.}  The clear positive impact from intervening in the intermediate layers [17-21] is demonstrated in the experimental group, in contrast to negligible effects observed in the control group across all layers. This suggests that the implicit subject $s_2$ at the last token position was used for retrieving the related information of $o_2$ from {\bf later MLP layers}. Thus, it plays an important role in the probability accumulation process of $o_2$. Note that this is in contrast with previous work~\citep{ROME,MEMIT}, which mentioned that explicit single-hop tasks primarily rely on the subject position token to retrieve information from {\bf earlier MLP layers}.


%However, compared to the previous work on single-hop tasks, our results demonstrate a significant difference.  
\begin{tcolorbox}[mydefinition={Takeaway 3}]
During the reasoning
process of the second-hop knowledge in two-hop scenarios, information related to the subject is used for retrieving relevant knowledge of the final answer from later MLP layers of the last token position, which is from the earlier MLP layers in single-hop cases. 
\end{tcolorbox}
\vspace{-0.1in}



==> ICLR_text/fig/larger_figure.tex <==

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\linewidth]{./pdf/2-hop_logitlens.pdf}
        \caption{Two-hop}
        \label{fig:two-hop-logitlens}
    \end{subfigure}
        \hfill
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\linewidth]{./pdf/1-hop_logitlens.pdf}
        \caption{Single-hop}
        \label{fig:larger_one-hop-logitlens}
    \end{subfigure}
    \caption{\textbf{LogitLens results of the last token position at different layers. } (a) \textcolor{logits-inter-a}{Yellow line} represents the information containing  implicit subject $s_2$, i.e., $\text{Info}(h_l,s_2)$. \textcolor{logits-final-a}{Blue line} represents the information for the final answer, i.e.,  $\text{Info}(h_l,o_2)$.  (b) \textcolor{logits-inter-a}{Yellow line} represents the information of subject $s$. i.e., $\text{Info}(h_l,s)$ and \textcolor{logits-final-a}{Blue line} represents the information of the answer $o$, i.e., $\text{Info}(h_l,o)$. Larger versions of the sub-figures are available in the Appendix} 
\end{figure}

==> ICLR_text/fig/mlp_llama.tex <==
\begin{figure*}[th]
  \centering
  \includegraphics[width=0.8\linewidth]{pdf/mlp_invemt_llama2.pdf}
  \caption{ Causal Intervention result of MLP hidden state in last token position on LLaMA-2}
  \label{fig:llama2_mlp_inter}
  \end{figure*}

==> ICLR_text/fig/teaser.tex <==
\definecolor{aaindex}{HTML}{000066}
\definecolor{support}{HTML}{DB8100}
\definecolor{orig}{HTML}{9F0000}
\definecolor{new}{HTML}{6600CC}
\begin{figure*}[th]
  \centering
  \includegraphics[width=1.0\linewidth]{pdf/Teaser_V2.0.pdf}
  \vspace{-0.2in}
  \captionsetup{skip=1pt}
  \caption{ \textcolor{aaindex}{\textbf{{(a)}}} The existing locate-then-edit KE method updates \textcolor{new}{\textbf{{new fact}}} to the shallow layers of the model using a single-hop edit template. \textcolor{aaindex}{\textbf{{(b)}}} For multi-hop fact recall tasks, especially when the edited fact is in the second or subsequent hops, the hops typically access the deeper layers which outputs the \textcolor{orig}{\textbf{{unmodified knowledge}}}. \textcolor{aaindex}{\textbf{{(c)}}} Our method introduces a \textcolor{support}{\textbf{{prefix hop}}} for each single-hop edit, creating a two-hop edit template. We utilize this new template to perform a furtherance edit, targeting the deeper layers for more effective knowledge updating.}
   \vspace{-0.25in}
  \label{fig:our-method}
  \end{figure*}
% \vspace{-0.3in}

==> ICLR_text/intro.tex <==
\vspace{-0.3in}
\section{Introduction}
\vspace{-0.1in}
Large Language Models (LLMs) like ChatGPT \citep{Achiam2023GPT4TR} and LLaMA-2 \citep{Touvron2023Llama2O} have emerged as powerful knowledge bases, demonstrating remarkable abilities in both factual knowledge representation and reasoning over complex queries \citep{Etezadi2022TheSO}. However, as the need for updating and correcting knowledge within these models grows, research on knowledge editing (KE) has gained significant attention, focusing on cost-effective ways to modify specific information in LLMs \citep{Mazzia2023ASO}. KE methods can be broadly classified into two categories based on whether they alter the original model weights: weight-preserving \citep{MQUAKE} and weight-modifying approaches \citep{ROME,meng2022mass}. Weight-preserving methods aim to modify the model's outputs by integrating external memory or leveraging strategies such as in-context learning without altering the underlying weights \citep{Cheng2024MultihopQA,cheng2024leveraging}. In contrast, weight-modifying methods directly change the model's internal weights to update the stored knowledge. Weight-modifying methods can be further categorized into learning-based and optimization-based methods. Learning-based methods update weights using gradients but face challenges such as overfitting and poor generalization. Optimization-based methods, such as ROME \citep{ROME} and MEMIT \citep{meng2022mass}, have introduced the ``locate-then-edit'' paradigm, which first identifies the knowledge storage layers and then adjusts their weights through optimization techniques to achieve the desired knowledge modification.

Compared to weight-preserving methods and learning-based weight-modifying approaches, the locate-then-edit paradigm offers precise editing of the model's internal knowledge with low computational costs~\citep{kesurvey}. However, despite the success of locate-then-edit methods in single-hop fact recall tasks~\citep{pmet}, they share a common limitation~\cite{MQUAKE}: \textbf{The post-edited model struggles with multi-hop factual recall tasks involving the newly edited knowledge} (see Table \ref{tab:main_result} for details). For example, after changing the knowledge ``The capital of Spain'' from ``Madrid'' to ``Hartford'', the model correctly answers \(Q_1 = \text{``What is the capital city of Spain?''}\). However, when posed with the multi-hop question \(Q_2 = \text{``What is the capital city of the country where Pablo Picasso holds citizenship?''}\), it still responds with ``Madrid'' (Figure \ref{fig:our-method} (b)). This discrepancy raises a natural question: \textit{Has the locate-then-edit approach reached its limits for multi-hop factual recall tasks, or does it still hold unexplored potential?}
\input{text/fig/teaser}

To answer this question, we first explored the mechanisms of the pre-edited model when handling single-hop and multi-hop factual recall tasks to gain insights. Using the example mentioned, we attempt to illustrate how the model reasons with the implicit subject ``Spain'' in \(Q_2\), compared to the explicit mention in \(Q_1\). We first use LogitLens \citep{LogitLens2020,logit-dar} to interpret the information encoded in each layer's hidden states by projecting them into the output vocabulary space. We find that at the last token position, the information of the implicit subject accumulates before the final answer, which is significantly different from the single-hop scenario. We then conduct causal intervention experiments~\citep{understand-li} to further confirm the influence of the implicit subject on the final answer.

Based on this, we further explore the mechanism of how the implicit subject influences the prediction of the final answer. By using causal intervention, our results indicate that in the multi-hop scenario, the implicit subject guides the emergence of the final answer by retrieving relevant knowledge from the {\bf later MLP layers}. This contrasts sharply with the single-hop cases~\citep{ROME,MEMIT}, where the subject information is used to retrieve information from {\bf earlier MLP layers}. Based on this difference, we provide an explanation for the unsatisfactory performance of the existing locate-then-edit methods for multi-hop tasks: Previous methods leveraging single-hop prompts for editing are insufficient as they only update the relevant knowledge in the shallow MLP layers but fail to propagate the changes to deeper layers. The model retains some of the old single-hop knowledge that only activated by additional implicit multi-hop fact recall mechanisms.

Based on these observations, we developed an advanced locate-then-edit KE method specifically designed to modify knowledge in both shallow and deep MLP layers, which we named \underline{\textbf{I}}nterpretability-Guided \underline{\textbf{F}}urtherance \underline{\textbf{M}}odel \underline{\textbf{E}}diting in a \underline{\textbf{T}}ransformer \textbf{(IFMET)}. IFMET introduces a supplementary set for edit instances and generates multi-hop editing prompts, surpassing the limitations of single-hop prompts used in previous locate-then-edit approaches. This supplementary set helps us locate pre-existing knowledge that appears in later hops by leveraging the differences between the reasoning mechanism for single-hop and multi-hop queries. By leveraging each edit instance and its corresponding multi-hop editing prompt, IFMET locates and edits the knowledge stored in both earlier and later MLP layers, effectively addressing cases where the knowledge to be edited appears either in the first or subsequent hops during reasoning, as illustrated in Figure~\ref{fig:our-method}.
Our contributions can be summarized as follows:
\setlength{\itemsep}{1pt}
\setlength{\parsep}{1pt} 
\setlength{\topsep}{0pt} % 列表顶部和第一个项目之间的间距
\begin{itemize}
    \item We first identified key differences in the mechanisms the model uses for reasoning in single-hop versus multi-hop fact recall tasks. In multi-hop scenarios, unlike single-hop cases, the model prioritizes inferring the implicit subject at the last token position, which guides the generation of the final answer.
    \item Next, we pinpointed the components of the implicit subject that influenced the final answer within the later MLP layers. We demonstrated that the absence of edited knowledge of these components significantly impacted the model’s performance.
    
    \item We propose IFMET, an advanced locate-then-edit KE method specifically designed to modify knowledge in both shallow and deep MLP layers using single and multi-hop edit prompts. Experimental results confirm the effectiveness of our method, showing that it successfully overcomes the limitations of previous locate-then-edit approaches in handling multi-hop factual recall tasks.
\end{itemize}
Due to the space limit, we refer readers to Appendix~\ref{sec:related} for previous work. 



==> ICLR_text/method.tex <==
\newcommand{\Km}[2]{\left[ k^1_{#1} \, \vert \, k^2_{#1} \, \vert \, \cdots \, \vert \, k^{#2}_{#1} \right]}
\newcommand{\Vm}[2]{\left[ v^1_{#1} \, \vert \, v^2_{#1} \, \vert \, \cdots \, \vert \, v^{#2}_{#1} \right]}
\newcommand{\Vmm}[2]{\left[ v^*_{#1} \, \vert \, v^*_{#1} \, \vert \, \cdots \, \vert \, v^{*}_{#1} \right]}

 \vspace{-0.15in}
\section{IFMET: An Advanced Locate-then-Edit Method }
\vspace{-10pt}
Motivated by our findings on the distinctions between single-hop and multi-hop factual recall process, we introduce the Interpretability-Guided Furtherance Model Editing in a Transformer (IFMET). This method addresses the limitations identified in existing locate-then-edit approaches by modifying knowledge across both earlier and later MLP layers, enhancing the model's ability to handle multi-hop reasoning. The IFMET method comprises two main steps: first, constructing a supplementary set of original edits to enrich the edit context, and second, performing editing based on multi-hop prompts derived from the original edit case and its supplementary set. This furtherance step approach ensures a thorough integration of new knowledge, significantly improving the model's accuracy and robustness in multi-hop factual recall scenarios.
\vspace{-1mm}
\begin{wraptable}{l}{0.5\columnwidth}
    \centering
    \setlength{\intextsep}{0pt} % 设置文本与wraptable环境的垂直距离为0pt
    \renewcommand{\arraystretch}{0.9} % 设置表格行距的缩放因子
    % \setlength{\abovecaptionskip}{-5pt} % 减小表格标题与表格之间的距离
    \setlength{\belowcaptionskip}{-8pt} % 减小表格与表格下方文字的距离
    \resizebox{0.48\columnwidth}{!}{
    \begin{tabular}{cl}
        \toprule
        $e$  & (Spain, capital, Madrid $\to$ Hartford) \\[1pt]
        $s$  & Spain \\[3pt]
        $T_r(s)$ & The capital city of Spain is\\[1pt]
        $C$ & (Manuel Almunia, citizenship, Spain) \\
        & (Spain, capital, Madrid $\to$ Hartford)\\[1pt]
        $Q_C(s)$ & What is the capital city of the country \\&
        where Manuel Almunia holds citizenship? \\
        \midrule
        $e'$ & (Barcelona, country, Spain) \\[1pt]
        $s'$ & Barcelona \\[1pt]
        $C'$ & \uwave{(Barcelona, country, Spain)} \\
        & (Spain, capital, Madrid $\to$ Hartford)\\[1pt]
        $T_C(s')$ & The capital city of the country \\&
        where Barcelona is located is \\
        \bottomrule
    \end{tabular}
    }
    \caption{An support case for an instance in the {MQuAKE-CF} dataset and the corresponding additional support cases are shown in the lower part.}
    \label{tab:support_example}
\end{wraptable}

\noindent {\bf Supplementary Set Construction.} Note that for a given edit $e = \left( s, r, o  \to  o^* \right)$ (it can be extended to cases involving multiple edited facts), a locate-then-edit algorithm typically aims to identify and modify the knowledge-storing MLPs. Previous efforts have predominantly focused on the earlier MLP layers; however, our findings indicate that such an approach underperforms when the edited knowledge appears in second or subsequent hops during reasoning. Given that each edit traditionally targets single-hop knowledge, our experiments have demonstrated that using such edit prompts alone does not effectively update the later knowledge-storing MLPs. To address this issue, we construct a supplementary set for each edit, designed to facilitate the modification of deeper MLPs that provide knowledge in implicit fact recall steps.

In our supplementary set, we transform each edit into a multi-hop chain. For instance, for an edit \(e = (s, r, o \to o^*)\), we can create a supplementary fact \(e_{\text{sup}} = (s', r', o')\) where \(o' = s\), forming a two-hop fact recall chain \(C = (s', r', o') \oplus (s, r, o)\). This approach enables us to subsequently target and modify the latter MLPs that store the fact \((s, r, o)\), updating the information to \((s, r, o^*)\). An illustrative example of this process is provided in Table \ref{tab:support_example}.

Practically, we utilize WikiData\footnote{www.wikidata.org} to construct the supplementary dataset. We start by extracting all subjects from the dataset's edits and deduplicating them to form a set of subjects \(S_e = \{s_i | i = 1, \dots\}\). We then perform a WikiData SPARQL query\footnote{https://query.wikidata.org/} to identify a set of triplets for each subject \(s_i\): \(Sup = \{(s', r', o') | o' = s_i\}\). To ensure the reliability of these facts, we filter out examples that cannot be correctly answered using the few-shot approach proposed by \citep{MQUAKE}. For construction details, please refer to the Appendix~\ref{a:construct-process}.


\noindent {\bf Interpretability-Enhanced Furtherance Model Editing in a Transformer.} Now we introduce the proposed IFMET framework. Each pre-edited knowledge has an additional multi-hop chain, assisted by the supplementary set. Based on the difference between the single and multi-top settings we discussed above, we have to locate and modify weights in both earlier and later layers in MLPs. 

%This framework integrates a furtherance editing process within the flow shaped by ROME~\cite{ROME}, sequentially performing edits of two types to achieve knowledge updates in both the shallow and deeper MLPs. 

Based on the previous key-value memories~\cite{memory_key_value}, our method is based on the hypothesis that factual knowledge is stored within the Feedforward Neural Networks (FFNs) of MLPs. Specifically, for the $l$-th layer FFN of the $i$-th token, its output is given by: $v^i_l = f(W^{in}_l h^i_{l-1})W^{out}_l$, where $f(\cdot)$ is the activation function, and $h^i_{l-1}$ is the input of the $l$-th MLP layer (for simplicity, the superscript $l$ is omitted in the
following discussion). In this context, $f(W^{in} h^i)$ functions as the keys, denoted as $k_i$, the outputs of the subsequent layer represent the corresponding values $v_i$, and \( W^{out} \) denotes the weights of the knowledge stored in the FFN that needs modifying.
Such a structure is well aligned with the triplet form in a fact $(s, r, o)$, where the keys $k_i$ correspond to entities of interest $s_i$ or some specific fact $(s_i,r_i)$ and values 
$v_i$ contain information about \( o_i \). Thus,  we have $W^{out}k = v$ for \((k,v)\), which represents the  fact $\left( s, r, o \right)$~\citep{memory_key_value}. We aim to modify $W^{out}$ such that $W^{out}k = v^*$, where $v^*$ contains the information of the new knowledge.


Motivated by the above, in IFMET,  considering a modification,  there are two steps for both earlier and latter layers in MLPs: \( Search \) and \( Calculate \). The \( Search \) process identifies the suitable \( v^* \) through the edit prompt corresponding to the triplet. Then the \( Calculate \) process computes the change in weights $W^{out}$ using \( v^* \). These two processes are foundational in existing knowledge editing methodologies. In experiments, we adopt the state-of-the-art locate-then-edit method PMET \citep{pmet}. The primary differences between the first and further edits are reflected in the edit prompt and the layers edited. Specifically, for the edit instance $e = (s,r,o \to o*)$, the first edit utilized a one-hop edit template $T_r(s)$ provided by MQuAKE to edit early layers of the model. For the furtherance edit, a two-hop template \( T_C(s') \) composed of a support case \((s',r,s)\) and \( (s,r,o^*) \) was used, and this template was applied to edit later layers of the model. Due to space limitations, the flowchart of the algorithm and related implementation details are provided in Algorithm~\ref{alg:mrome} and Appendix ~\ref{a:construct-process}.


==> ICLR_text/method_orig.tex <==
% \newcommand{\Km}[2]{\left[ k_1^{#1} \, \vert \, k_2^{#1} \, \vert \, \cdots \, \vert \, k_{#2}^{#1} \right]}
% \newcommand{\Vm}[2]{\left[ v_1^{#1} \, \vert \, v_2^{#1} \, \vert \, \cdots \, \vert \, v_{#2}^{#1} \right]}
\section{Enhanced Existing Knowledge Editing \di{CHnage the title}}
% Single case in the knowledge editing task can be simply summarized as following quadruple: \( p(s, r), o, o^*, p_{\text{test}} \), where $p(s,r)$ is the Cloze-Format prompt used for editing the knowledge. $o$ and $o^*$ represent the original and new object, respectively. And \( p_{\text{test}} \) denotes the prompt used to test different type of performance of editing method. It may either be the same or a rephrasing of \( p(s, r) \), or it could involve other subjects sharing the same relation $p(s_r,r)$. And The whole set with multiple knowledge editing cases denoted as 
% $
% \{(p(s_i, r_i), o_i, o_i^*, p_{\text{test},i}) \mid i = 1, 2, \dots, E\},
% $
% where each element follows the same structure. \di{No, this should be included in  preliminaries, not here}


% \subsection{Unified Framework of existing methods} 
% \di{The whole section is about previous method, I think you should move to preliminaries. }
% Following previous work, we adopt a unified framework to explore locate-then-edit methods. We demonstrate that approaches like ROME, MEMIT, PMET, and EMMET are variations of this framework. 

% \noindent {\bf Preserve-Edit Objective } Like \cite{memory_key_value} and \cite{ROME}, we treat the Feed-Forward Network(FFN) as a key-value store for knowledge. Let \( W_0 \) denote the original weights of the FFN that needs modifying. The \( k \), input vector of $W_0$, acting as a lookup \textbf{key}, represents entities of interest $s$ or some specific fact $(s,r)$. The hidden states produced after passing through the FFN are treated as \textbf{values} \( v \), which represent the knowledge associated with \( k \), retrieved from the weights \( W \). And \( v\) is typically considered to contain information about \( o \). So that a \((k,v)\) pairs, satisfying $Wk = v$, represent the full fact $\left( s, r, o \right)$. After Knowledge Editing, the weights of FFN are changed from $W_0$ to $W_e$ , we can define the objective of knowledge preservation and editing:
% \[
% \underbrace{\mathbf{P}(\hat{W},K_0,V_0)}_{\text{Preserve}}
% \quad \text{and} \quad
% \underbrace{\mathbf{E}(\hat{W},K_e,V_e)}_{\text{Edit}}
% \]
% Where $K_0 = \Km{0}{N}$ and $V_0 =  W_0 K_0$ containing all the knowledge we want to preserve in a row. $K_E = \Km{e}{E}$ is a matrix containing the edits we try to make and $V_e = \Vm{e}{E}$ represents the target representations of the new knowledge. ($K_E,V_E$) corresponds to the edited fact set  $\{\left( s_i, r_i, o^*_i \right) \vert i = 1,2,\cdots,E\}$. The differences between these existing methods lie in the selection of the preservation objective $\mathbf{P}$ and the editing objective $\mathbf{E}$. For instance, if we use least squares method to constrain both the preservation and edit, we obtain MEMIT: 
% \[
% \argmin_{\hat{W}} \left( \lambda \underbrace{\| \hat{W} K_0 - W_0 K_0 \|^2}_{\text{Preserve}} + \underbrace{\| \hat{W} K_E - V_E \|^2}_{\text{Edit}} \right)
% \]

% Different types of constraints lead to different optimization methods, but ultimately yield solutions of similar form: $ \hat{W} = W_0 + \Delta$ where $\Delta$ is a function of $W_0, V_E,  K_E$. Specific functions used to compute $\Delta$ and more optimization objectives of other methods refer to the Appendix.

% \noindent {\bf FFN selection and Edit-Layer-Propagation Algorithms } Through causal tracing methods, these method select the second FFN in MLP as the target to edit knowledge. When find the $V_E$, they propagate the desired updates of \textbf{values} vector $R = V_E-W_0K_E$ across all the critical layers. We refer to this algorithm as an \textbf{Edit-Layer-Propagation Algorithms}, applied post-hoc after finding the closed-form solutions to the PE-objective. This has contributed to the outstanding performance of MEMIT and PMET in editing tasks, particularly with large batch sizes. 

% \noindent {\bf  Target value vector of the new knowledge } To obtain the target \textbf{values} vector of the new knowledge $V_E$, these methods use an objective function based on KL divergence and maximizing $\mathbb{P}[o^*|p(s,r)]$, the output probability of the edited knowledge in prediction layer. For further details, please refer to the Appendix.

% \subsection{IDMET method}

% \noindent {\bf Interpretable Edit-Layer-Propagation Algorithm } As we observed in \ref{components}, each individual MLP contributes by \textit{adding} to related knowledge at specific tokens, which is later read by last-token attention modules, and the related knowledge is gradually accumulated over layers. Thus, \cite{MEMIT} propose using the \textbf{Edit-Layer-Propagation Algorithm} to achieve more effective knowledge transfer. Let $A$ represent the weight matrix for propagation between layer $i$ and layer $j$, $A = [f_{ij}]$ with $f_{ij} = g(i, j)$. Compared to MEMIT's use of even distribution $g(i, j)=\frac{1}{j-i+1}$, PMET employs $g(i, j)=\frac{1}{\sqrt{j-i+1}}$ to transmit more precise information to the critical layers. However, these algorithms function more like a hyperparameter and lack interpretability. Given that the circuit's edges model the influence of one component's output on another, they can be effectively applied it to optimize edge propagation algorithms, wthich we called  Interpretable Edit-Layer-Propagation Algorithm(IEPA). \di{Why you are still introducing previous method? }


% \noindent {\bf Furtherance Editing For Multi-hop} 


% \setlength{\algomargin}{10pt}
% \RestyleAlgo{ruled}
% \newlength{\commentWidth}
% \setlength{\commentWidth}{7cm}
% \newcommand{\atcp}[1]{\tcp*[f]{\makebox[\commentWidth]{#1\hfill}}}
% \newcommand{\atcpl}[1]{\tcp*[r]{\makebox[\commentWidth]{#1\hfill}}}
% \newcommand\mycommfont[1]{\footnotesize\textcolor{blue}{#1}}
% \newcommand{\elid}[2]{#1_{#2}}
% \newcommand{\tresid}{\elid{\delta}{i}}
% \newcommand{\prsub}[2]{\mathbb{P}_{#2}\left[ #1 \right]}
% \newcommand{\atl}[2]{#1^{#2}}
% \newcommand{\refeqn}[1]{Eqn.~\ref{eq:#1}}
% \newcommand{\method}{MEMIT\xspace}
% \newcommand{\Gsub}{G(\atl{h}{L}_i\mathrel{+}=\tresid)}
% \SetCommentSty{mycommfont}
% \begin{center}
% % \scalebox{0.9}{
% \begin{minipage}{\linewidth}
% \begin{algorithm}[H]
% \SetAlgoLined
% \caption{The IDMET Algorithm}\label{alg:mrome}
% \KwData{Requested edits $\mathcal{E} = \{ (s_i, r_i, o_i) \}$, generator $G$, layers to edit $\mathcal{S}$, covariances $C^l$}
% \KwResult{Modified generator containing edits from $\mathcal{E}$}

% \For(\quad \atcp{Compute target $z_i$ vectors for every memory $i$}){$s_i, r_i, o_i \in \mathcal{E}$}{
%     \textbf{optimize} $\delta_i \leftarrow \argmin_{\delta_i    } \frac{1}{P} \sum_{j=1}^P -\log\prsub{o_i \mid x_j \oplus p(s_i, r_i)}{\Gsub}$ (\refeqn{compute-z}) \;
%     $z_i \gets \atl{h}{L}_i + \delta_i$ \;
% }
% \For(\quad \atcp{Perform update: spread changes over layers}){$l \in \mathcal{R}$}{
%     $\atl{h}{l}_i \gets \atl{h}{l-1}_i + \atl{a}{l}_i + \atl{m}{l}_i$ (\refeqn{autoregressive}) \quad \atcpl{Run layer $l$ with updated weights}
    
%     \For{$s_i, r_i, o_i \in \mathcal{E}$}{
%         $k^l_i \gets \atl{k}{l}_i = \frac{1}{P} \sum_{j=1}^P k(x_j + s_i)$ (\refeqn{compute-k}) \;
%         $r^l_i \gets \frac{z_i - \atl{h}{L}_i}{L - l + 1}$ (\refeqn{compute-v}) \quad \atcpl{Distribute residual over remaining layers}
%     }
%     $K^l \gets$ \texttt{[$k^{l_1}_i, ... ,k^{L}_i$]}  \quad \atcpl{Update }
%     $R^l \gets$ \texttt{[$r^{l_1}_i, ... ,r^{L}_i$]} \;
%     $\Delta^l \gets R^l {K^l}^T (C^l + K^l {K^l}^T)^{-1}$ (\refeqn{multirome-update})   \;
%     $W^l \gets W^l + \Delta^l$ \quad \atcpl{Update layer $l$ MLP weights in model}
% }
% \end{algorithm}%
% \end{minipage}%
% % }%
% \end{center}



==> ICLR_text/prelim.tex <==
\vspace{-10pt}
\section{Preliminaries}
 \vspace{-0.1in}
{\bf Notations.} We define the set of knowledge as $\mathcal{K}=\{( s, r, o)\} \subseteq \mathcal{E} \times \mathcal{R} \times \mathcal{E}$, where $\mathcal{E}$ and $\mathcal{R}$ denote the set of entities and relations respectively. Each tuple $(s,r,o) \in \mathcal{K}$ represents that the corresponding entity of subject entity $s$ under relation $r$ is object entity $o$. An editing instance can be described in the form of a triplet: $e = \left( s, r, o  \to  o^* \right)$, where $o^*$ denotes the new edited object in place of the original object $o$ related to $s$ through $r$. %\textbf{In existing knowledge editing methods, the corresponding Cloze-style single-hop prompt $T_r(s)$ is typically used for performing the edit in shallow MLPs.} 

\textit{Multi-hop factual recall} $Q$ requires multi-step reasoning to reach the final answer. Its reasoning process is composed of a chain of knowledge $C = \left( s_1, r_1, o_1 \right) \oplus \dots \oplus \left( s_n, r_n, o_n \right) $, where $s_1$ is the start subject that is explicitly given in the question, $o_n$ is the final answer, and $\oplus$ used for chain adjacent reasoning steps which means the subject $s_{i+1}$ is identical to the object $o_i$ of preceding reasoning step. In order to better explore how the language model recalls multi-hop questions, we categorize the reasoning step into two types: \textit{explicit recall step} $(s_1,r_1,o_1)$ and \textit{implicit recall steps} $ \{ \left( s_2, r_2, o_2\right),\dots, \left( s_n, r_n, o_n \right)\}$. The inference information required by the former subject $s_1$ explicitly appears in the prompt, while the subjects of the latter $s_2...s_n$ need to be inferred to obtain, which are called implicit subjects. 

 \vspace{-0.15in}
\subsection{Factual Recall Tasks}
 \vspace{-0.1in}
\noindent {\bf Format of Factual Recall Tasks.}
Factual recall tasks refer to verifying whether the model $\mathcal{M}$ can correctly provide the final answer to a single-hop question or a multi-hop factual recall $Q$. Based on the two forms of declarative sentences and interrogative sentences, there are two different formats of factual recall tasks: Cloze-Format $Q_{cloze}$ and QA-Format $Q_{qa}$. For instance, given two-hop questions with the knowledge chain like \textit{(Paradiso, author, Dante Alighieri)} $\oplus$ \textit{(Dante Alighieri, country of citizenship, Italy)}, $Q_{cloze}$ can be ``The author of Paradiso is a citizen of'', while $Q_{qa}$ is ``What country does the author of Paradiso hold citizenship in?''. If the model's final answer is the same as the answer to the question, the recall is considered successful, which can be represented as $\mathcal{M}(Q_{cloze}) = o_n$ or $\mathcal{M}(Q_{qa}) = o_n$.


\noindent {\bf Multi-hop Factual Recall under Knowledge Editing.} This task assesses whether the post-edited model can effectively leverage the updated knowledge for reasoning in multi-hop fact recall tasks. Given an edit $e = \left( s, r, o  \to  o^* \right)$, the edit prompt $T_r(s)$ and a chain of facts $C_e$ which includes $\left( s, r, o \right)$ as one of its components. After the post-edited model must leverage the new factual knowledge $\left( s, r, o^* \right)$ to answer the multi-hop query. For example, given edit \textit{(Paradiso, author, Dante Alighieri $\to$ Mark Twain)}, the model’s response of ``The author of Paradiso is a citizen of'' should change from the original answer \textit{Italy} to the new answer \textit{USA}.

\vspace{-0.1in}
\subsection{Mechanistic Interpretation Tools}

\noindent {\bf LogitLens.}
\label{LogitLens} 
LogitLens \citep{LogitLens2020} is a framework for interpreting the hidden states (activations) of language models such as GPT~\citep{few_shot_1} by examining the logits (the raw prediction scores before they are transformed into probabilities) and corresponding probabilities. Specifically, for the hidden state \(h^i_l\) at the \(l\)-th layer and position \(i\), the logits \(s^i_l\) and probabilities \(p^i_l\) over the output vocabulary set \(V\) are defined as follows:
\[
\begin{cases} 
     s^i_l = W_U h^i_l \in \mathbb{R}^{|V|}, \\
     p^i_l = \text{softmax}\left(s^i_l\right)
\end{cases}
\]
% 
where \(W_U\) denotes the unembedding matrix, which is the same matrix used in the final layer of the model for prediction. LogitLens aids in the decomposition of model predictions, elucidating the contributions from various input components such as MLPs and attention heads. This decomposition can be explored by modifying \(h^i_l\) to the output from MLP \(m^i_l\) or attention heads \(a^i_l\), where \(h^i_l = h^{l-1}_i + m^i_l + a^i_l\). \footnote{We employ GPT variants such as GPT-J~\cite{GPT-J} that position attention in parallel to the MLP, which mathematically equates to models that calculate MLP sequentially after the attention module, as discussed in \cite{few_shot_1}.} LogitLens posits that probabilities and logits provide insights into how the model prioritizes different potential tokens, as indicated by the proportion of related information. Specifically, we define \(\text{Info}(h^i_l,j)\) as the information related to token \(j \in V\) contained in \(h^i_l\), positively correlated with \(s^i_l[j]\) and \(p^i_l[j]\). To account for the probability variations across different layers, we define \(\text{Info}(h^i_l,j)\) as the layer-wise min-max normalized probability~\citep{understand-li}, where \(L\) is the total number of layers:
\[
\begin{cases} 
     p^i_{max}[j] = \max\limits_{\{l = 1, \ldots, L\}} p^i_l[j],\\
     p^i_{min}[j] = \min\limits_{\{l = 1, \ldots, L\}} p^i_l[j],\\
     \text{Info}(h^i_l,j) = \frac{p^i_l[j]-p^i_{min}[j]}{p^i_{max}[j]-p^i_{min}[j]}
\end{cases}
\]

\noindent {\bf Causal Intervention on Hidden States.}
\label{CausalIntervention} 
Causal intervention on hidden states~\cite{understand-li,li2024intervent} involves deliberately altering specific hidden states in a model to observe the resulting changes in various metrics, thereby helping to establish cause-and-effect relationships. This process includes three pivotal components: the intervention operation \(\mathcal{I}\) to be conducted, the target hidden state \(\mathcal{H}\) selected for intervention, and the effect metric \(\textit{IE}\) which measures the change caused by the intervention \(\mathcal{I}\). In this paper, the possible hidden states \(\mathcal{H}\) for intervention include the layer hidden states \(h\), the output hidden states from MLPs \(m\), and the output hidden states from attention heads \(a\). We use the change in probability \(p^{i}_{l}[j]\) from LogitLens as the effect metric \(\textit{IE}\), which quantifies the change in the probability of predicting the target token \(j\) at layer \(l\) for a specific position \(i\). This metric enables us to determine whether specific components or tokens, have a causal influence on the model's predictions.


==> ICLR_text/rebuttal.tex <==
\noindent {\bf Official Review of Submission3638 by Reviewer Pi7C}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item For Q1, We have widened Figures 2(a) and 2(b) and enlarged the subfigures in Figure 7(Figure 6 in previous version) to improve visibility.
    \item For weakness 1,2 and Q2, We revised the terminology in Tables and Figures, to consistently refer to the unmodified model as "Base". Additionally, we included a unified explanation of this term in the \textbf{Baseline} section of \textbf{5.1 Experimental Setup}. Then We provided detailed explanations of the reported outcomes in tables in the \textbf{Setup and Hyperparameters section} of \textbf{5.1 Experimental Setup}, ensuring consistent definitions for \textbf{"original answer"} and \textbf{"edited answer".} Notes have also been added below each table to clarify the meaning of these values. We hope this explaination address your concerns about Questionable Analysis of Results in Table 3 and others.
    \item For weakness 3 To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. Importantly, they confirm that the observed performance improvements are not solely attributable to the supplementary set.
\end{enumerate}
Regarding the organization of the paper, we fully understand the difficulties you encountered when important results were placed in the appendix. We spent considerable time attempting to incorporate more tables into the main text but were ultimately unsuccessful. At the same time, we believe that the analytical section preceding the experiments is necessary. Therefore, we kindly ask for your understanding that due to space constraints, we had to place some tables, and even the entire ablation study, in the appendix. Our aim was to preserve the completeness of the experimental results as much as possible. All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer 1m6u}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item We have corrected the typo errors you mentioned(Line 387, cizizenship $\rightarrow$ citizenship, Figure 1, Mardrid $\rightarrow$ Madrid.) and The biblology style has been consistent.
    \item Ablation study Analyses: To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position.
    \item For weakness 1, we first extended the causal intervention experiments to the LLaMA2-7B model, demonstrating the consistency of interpretability analysis while validating the effectiveness of our method. You can check it in Figure 6 and Table 9 in new version.
    \item For wakness 2: We constructed the paraphrase set and neighborhood set for a subset of the MQuAKE-CF dataset, following the approach used in the COUNTERFACT dataset. The results indicate that IFMET outperforms single-stage editing methods (PMET) in Multi-hop Accuracy, Efficacy Score, and Paraphrase Score, with only a minor decrease in the Neighborhood Score. For more details on related ablation studies, please refer to the corresponding section.
    \item For weakness 3: We compared the time complexity of \textbf{IFMET} with that of the one-stage \textbf{PMET} method it builds upon. On average,the time required to perform a complete edit for a single case on GPT-J using \textbf{IFMET} was approximately 2.5$\times$ that of \textbf{PMET}. For LLaMA-2, the time required was about 1.5$\times$ that of \textbf{PMET}. We believe this is within an acceptable range, and as the editing speed of the single-stage method improves, the \textbf{IFMET} framework will correspondingly become faster.
    \item For weakness 4: we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Construction of the supplementary set}, providing a detailed explanation on utilizing the model itself to generate the supplementary set.
    \item The application of IFMET to unstructured knowledge editing presents a compelling avenue for further research. Unstructured text inherently encompasses more complex semantic information, and in scenarios involving longer and more intricate texts, the presence of noise can significantly complicate the reasoning process. At present, combining \textbf{IFMET} with efficient fact triple extraction techniques appears to be a feasible approach. We believe this context warrants deeper investigation in future work.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer bAUb}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item Ablation study and Generalizability Analyses: To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. And we discuss the generalizability of our method in many perspectives
    \item For discussion on why IFMET is superior to these RAG-based methods: we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Comparison with Weight-Preserving Methods}, providing a detailed explanation on why we try to explore the potential of locate-then-edit approach.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer ocTZ}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item For weakness 1, we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Construction of the supplementary set}, providing a detailed explanation on utilizing the model itself to generate the supplementary set.
    \item For weakness 2, We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. And we discuss the generalizability of our method in many perspectives
    \item For weakness 3, We revised the terminology in Tables and Figures, to consistently refer to the unmodified model as "Base". Additionally, we included a unified explanation of this term in the \textbf{Baseline} section of \textbf{5.1 Experimental Setup}. Then We provided detailed explanations of the reported outcomes in tables in the \textbf{Setup and Hyperparameters section} of \textbf{5.1 Experimental Setup}, ensuring consistent definitions for \textbf{"original answer"} and \textbf{"edited answer".} Notes have also been added below each table to clarify the meaning of these values. We hope this explaination address your concerns about Questionable Analysis of Results in Table 3 and others.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.
Regarding the organization of the paper, we fully understand the difficulties you encountered when important results were placed in the appendix. We spent considerable time attempting to incorporate more tables into the main text but were ultimately unsuccessful. At the same time, we believe that the analytical section preceding the experiments is necessary. Therefore, we kindly ask for your understanding that due to space constraints, we had to place some tables, and even the entire ablation study, in the appendix. Our aim was to preserve the completeness of the experimental results as much as possible.


==> ICLR_text/related.tex <==
\section{Related Work}\label{sec:related}
\noindent {\bf  Parameter-based Editing}
% ROME, explores the knowledge storage mechanism in single-hop factual recall tasks based on Causal Tracing methods and proposes the Rank-One Model Editing method. Together with KN, ROME pioneered the edit paradigm of first locating and then modifying the knowledge, known as \emph{locate-then-edit}. Subsequent methods, MEMIT and EMMET, further improved upon ROME by enabling large-scale edits to be performed in a single operation, demonstrating impressive editing performance. PMET, on the other hand, achieved more precise parameter modifications by decoupling the transformer’s residual stream into three parts: Multi-Head SelfAttention (MHSA), FFN, and residual connections. 
Knowledge editing refers to modifying outdated, inaccurate, or harmful knowledge in LLMs without the need for retraining. Parameter-editing methods achieve this by adjusting the model's internal parameters to update its knowledge while ensuring that information unrelated to the editing domain remains unaffected. An example is ROME \citep{ROME}, which explored the knowledge storage mechanisms in single-hop factual recall tasks based on causal tracing methods and proposed the Rank-One Model Editing method. Together with KN \citep{KN}, it pioneered a paradigm of \emph{locate-then-edit}, providing guidance for subsequent editing methods. The later extended versions, MEMIT \citep{MEMIT}, MALMEN \citep{MALMEN}, and EMMET \citep{EMMET}, further improved ROME by addressing its limitations in large-scale editing, enabling comprehensive edits in a single operation while demonstrating exceptional performance. Meanwhile, PMET \citep{pmet} achieved more precise model editing by decoupling the residual flow of the Transformer into three components: Multi-Head Self-Attention (MHSA), Feed-Forward Networks (FFN), and residual connections, utilizing only the optimized hidden states of the FFN to accurately update FFN weights. Additionally, MEND \citep{MEND} trained a hypernetwork to efficiently predict LLM weight updates, enabling rapid knowledge editing. METO \citep{METO} optimized the model’s temporal prediction of facts, editing both historical and new knowledge to reduce forgetting during updates. Wilke \citep{Wilke} selected the layers in LLMs that best matched the knowledge pattern for editing, achieving continuous updates and corrections in the model’s knowledge. \citet{Mece} used canonical examples to guide the model editing process, enabling fine-tuned adjustments to model behavior. However, these editing methods primarily focus on knowledge updates in specific layers and lack in-depth optimization for knowledge integration and application in multi-hop reasoning, rendering them inadequate for multi-hop questions. In contrast, IFMET enhances model interpretability, guiding more accurate knowledge integration and thereby improving model performance in multi-hop factual recall tasks.

\noindent {\bf Mechanistic Interpretability}
LLMs are capable of producing high-quality answers, but their internal workings remain opaque. As a result, the interpretability of LLMs has emerged as both a research hotspot and a critical area of focus. Mechanistic Interpretability refers to the effort to explain the internal mechanisms, decision-making processes, and outputs of LLMs. There are two primary approaches for interpreting large language models (LLMs) in the vocabulary space by examining hidden representations: Probing Classifiers \citep{belinkov2019analysis,belinkov2022probing,wang2024gaussian} and Projecting Representations to the Vocabulary Space \citep{dar2022analyzing,merullo2023mechanism,belrose2023eliciting,langedijk2023decoderlens}. The former identifies which parts of the model are crucial for specific tasks by training classifiers, known as probes, on hidden representations, while the latter involves mapping intermediate layer representations to the output vocabulary space and analyzing how these projections predict the next word.  In this paper, we focus primarily on Projecting Representations. Logit Lens \citep{LogitLens2020} extracted outputs corresponding to each layer in the decoding space by applying unembedding operations on the intermediate layers of LLMs. \citet{geva-etal-2022-transformer} analyzed the nature of updates at each layer by comparing differences in logit outputs. \citet{merullo2024languagemodelsimplementsimple} used the Logit Lens to explore how LLMs handle different stages of question-answering tasks. \citet{dar2022analyzing} mapped attention weights of LLMs to lexical space, showing that these weights encode consistent concepts and relations. \citet{belrose2023eliciting} introduced the Tuned Lens, which improves the capability and reliability of the Logit Lens. Finally, \citet{ghandeharioun2024patchscope} proposed the Patchscopes framework, demonstrating that auxiliary models can represent lexical projections through tuning. 

Mechanistic Interpretability serves as a tool for debugging and enhancing LLMs and can be applied to a variety of downstream tasks. \citet{xiao2024efficientstreaminglanguagemodels} leveraged explanations from multi-head self-attention (MHSA) mechanisms in LLMs by introducing StreamingLLM, a model capable of handling unlimited text without requiring fine-tuning. Through causal tracing, \citet{hendel2023incontextlearningcreatestask,todd2024functionvectorslargelanguage} demonstrated that certain attention heads can efficiently encode compact representations of example tasks, leading to improved performance in few-shot prompting. \citet{dev} explored the role of social bias in LLMs, introducing the concept of social bias neurons to explain and mitigate such biases. Furthermore, \citet{li2024inferencetimeinterventionelicitingtruthful} proposed an intervention technique during inference, which, based on the interpretability of attention heads, shifts activation values toward ``truthful" responses to reduce model hallucinations. In this paper, we analyze the MLP and MHSA components of LLMs to uncover the mechanisms that enable multi-hop reasoning,and building on our findings, we introduce a targeted knowledge-editing method IFMET.



==> ICLR_text/results/ablation_3000.tex <==
\begin{table*}[t]
\centering
\resizebox{0.65\textwidth}{!}{ 
  \centering
     \begin{tabular}{lcllllll}
    \toprule
        \multicolumn{1}{c}{\textbf{Edits}}&\multicolumn{1}{c}{\textbf{Editor}} & \multicolumn{1}{c}{\textbf{Multi-hop Acc} }& \multicolumn{1}{c}{\textbf{Efficacy} } \\
        \midrule
\multirow{6}{*}{3000}
&IFMET & {\textbf{17.40} \goodmetric{($\uparrow$48.7\%)}} &{94.74} ($\uparrow$0.1\%)  \\
&\makecell{w/o $First$} & {15.50} ($\uparrow$32.4\%) & {54.15} (\badmetric{$\downarrow$42.8\%})  \\
&\makecell{w/o $Sup$} & {11.33} (\badmetric{$\downarrow$3.2\%}) & {98.90} \goodmetric{($\uparrow$4.5\%)}  \\
&\makecell{w/o $Last$} & {12.90} ($\uparrow$10.2\%) & {94.69} ($\downarrow$0.1\%) \\ 
&\makecell{w/o $Deeper$} & {12.33} ($\uparrow$5.3\%) & {93.45} ($\downarrow$1.2\%) \\
&PMET & {{11.70}} &{{94.62}} \\ 
% &PMET & {{11.70} ($\downarrow$32.8\%)} &{{94.62} ($\downarrow$0.1\%)} \\ 
    \bottomrule
    \end{tabular}
    }
 \caption{The results of the ablation experiments of MQuAKE-3K on GPT-J-6B model. \textbf{w/o $First$} represents only optimizing the deeper MLPs with $Sup$ without modifying shallow MLPs first. 
 \textbf{w/o $Sup$} represents reusing Single-hop rewrite query used in first stage rather than the $Sup$ queries to modify deeper MLPs. \textbf{w/o $Last$} represents second stage editing occured in subject last token position.  \textbf{w/o $Deeper$} represents apply second stage editing in shallow MLPs. \textbf{PMET} represents the original one-stage method we used. Both the percentages of decrease($\downarrow$) and increase($\uparrow$) are calculated relative to \textbf{PMET} as the baseline. The most significant performance decline is highlighted in \badmetric{red} and the most significant performance increase is highlighted in \goodmetric{green}.
}
 \label{tab:ablation_3000}
 \end{table*}

==> ICLR_text/results/edit_num_table.tex <==
 % 设置表格内字体命令
\begin{table}[htbp]
    \centering
    \resizebox{0.8\textwidth}{!}
    {  % 调整表格宽度到页面宽度，高度自适应
    \renewcommand{\arraystretch}{1.2}  % 设置行间距
    \begin{tabular}{l l c c c c c}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Average Accuracy} & \textbf{1-Edit} & \textbf{2-Edit} & \textbf{3-Edit}& \textbf{4-Edit} \\
        \midrule
                
        \multirow{8}{*}{GPT-J-6B} & {Base} & 42.83 & 36.96 & 45.27& 46.85 &48.51\\
         \cmidrule(lr){2-7}  % 在MEND和IKE之间插入横线
                                        & {FT} & 1.9 & 4.2 & 0.7 & 0.3 &0.0 \\
                                        & {MEND} & 11.5 & 16.0 & 11.0& 7.3&4.4 \\
                                        & {ROME}  & 18.1 & 23.8 & 20.9& 9.0&2.6\\
                                        & {MEMIT}  & 12.3 & 20.5 & 9.8& 5.5 &2.6\\
                                        & {PMET}  & 17.04 & 22.63 & 16.74& 11.19& 7.84\\
                                        & \textbf{IFMET (ours)} & \bftab{31.01} & \bftab{30.26} & \bftab{35.21} & \bftab{24.30}& \bftab{31.72}\\
        \bottomrule
    \end{tabular}
    }
     \caption{\rebuttal{\textbf{Multi-hop Acc} Performance comparing the baselineand our method  with CoT on  multi-hop questions in MQuAKE-3k, categorized by the number of edits {1, 2, 3, 4}. \textbf{Base} in this table represents unmodified GPT-J-6B model, and we report its performance on \textbf{unedited answer} with CoT.}} 
    \label{tab:edit_result}
\end{table}

\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/Batch_size.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/hop_zhexian.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/edit-zhexian.pdf}
    \end{minipage}
    \caption{\rebuttal{\textbf{Multi-hop Acc} Performance Comparison of different methods across batch sizes, hop numbers, and edit instances. \textbf{Base} in this table represents unmodified GPT-J-6B model, and we report its performance on \textbf{unedited answer} with CoT.}}
    \label{fig:comparison_of_methods}
\end{figure}



==> ICLR_text/results/hop_num_table.tex <==
% 设置表格内字体命令

\begin{table}[htbp]
    \centering
    \resizebox{0.8\textwidth}{!}
    {  % 调整表格宽度到页面宽度，高度自适应
    \renewcommand{\arraystretch}{1.2}  % 设置行间距
    \begin{tabular}{l l c c c c}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Average Accuracy} & \textbf{2-hop} & \textbf{3-hop} & \textbf{4-hop} \\
        \midrule
                
        \multirow{8}{*}{GPT-J-6B} & {Base} & 42.83 & 48.9 &30.7& 48.9\\
         \cmidrule(lr){2-6}  % 在MEND和IKE之间插入横线
                                        & {FT} & 1.9 & 3.7 & 1.4 & 0.5 \\
                                        & {MEND} & 11.5 & 13.9 & 11.3& 9.5 \\
                                        & {ROME}  & 18.1 & 33.8 & 9.1& 11.4\\
                                        & {MEMIT}  & 12.3 & 22.5 & 6.0& 8.4 \\
                                        & {PMET}  & 17.04 & 26.65 & 12.76&11.7\\
                                        & \textbf{IFMET (ours)} & \bftab{31.01} & \bftab{44.06} & \bftab{23.58} & \bftab{25.4}\\
        \bottomrule
    \end{tabular}
    }
    \caption{\rebuttal{\textbf{Multi-hop Acc} Performance comparing the baseline and our method with CoT on multi-hop questions in MQuAKE-3k, categorized by hop counts of {2, 3, 4}. \textbf{Base} in this table represents unmodified GPT-J-6B model, and we report its performance on \textbf{unedited answer} with CoT.} }
    \label{tab:hop_result}
\end{table}



==> ICLR_text/results/main_ablation.tex <==
% 设置表格内字体命令


% \newcommand{\cellgray}{\cellcolor[gray]{0.9}}   % 定义浅灰色背景
% \newcommand{\good}[1]{\textbf{#1}}        % 方便表示加粗文本
% \begin{table}[!ht]
%     \centering
%     \renewcommand{\arraystretch}{1.2}  % 调整行间距
%     \resizebox{\textwidth}{!}{ 
%     \begin{tabular}{|l|c|c c c|c|c c c|}  % 创建表格布局，调整列格式
%         \toprule
%         \multirow{2}{*}{\textbf{Editor}} & \multicolumn{4}{c|}{\textbf{Correct Answer $\uparrow$}} & \multicolumn{4}{c|}{\textbf{Original Answer $\downarrow$}} \\ 
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%         & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} \\
%         \midrule

        
%         GPT-J       & 7.70 & 6.03 &16.92&7.00&39.63&38.43&35.9&44.27 \\ 
%         GPT-J+{CoT}       & 6.83 & 5.92 &9.23&7.76&42.83&41.56&39.74&47.33 \\ \cmidrule(lr){2-9}
%         PMET        &11.17& 12.13 & 16.09 &6.52&29.95&23.60&35.66&41.85 \\ 
%         PMET+{CoT}  & 17.04 & 19.84 &14.32&11.91&29.35&23.12&\good{30.43}&43.22 \\ 
%         IFMET       &23.04& 20.24 & 15.28 &33.38&23.08&20.18&34.32&\good{24.25} \\
%         \cellgray \textbf{IFMET+{CoT}} & \cellgray \good{31.01} & \cellgray \good{31.69} & \cellgray \good{19.49} & \cellgray \good{35.15} & \cellgray \good{21.62} & \cellgray \good{17.71} & \cellgray 30.51 & \cellgray 26.27 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance comparison between correct and original answers using PMET and our editors, with an edit batch size of 1. The type of edited fact—Pre, Mid, or Post—depends on the edited data position within the multi-hop reasoning chain. Average accuracy is calculated as the weighted average of results from these three categories, which have respective quantities of 1824, 390, and 786. Additionally,  +CoT denoted the performance incorporating a Chain-of-thought (CoT) prompt,  which can significantly enhance model performance for reasoning tasks. }
%     \label{tab:main_ablation}
% \end{table}
% \vspace{-0.05in}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \renewcommand{\arraystretch}{1.5}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{ 
\begin{tabular}{cccccccc}
\toprule
\multicolumn{3}{c}{\textbf{One-Stage Edit}}                                            & \multicolumn{3}{c}{\textbf{Two-Stage Edit}}                                 & \textbf{Multi-hop Acc} & \textbf{Efficacy} \\ \midrule
\textbf{Data}               & \textbf{Layers}          & \textbf{Position}             & \textbf{Data}               & \textbf{Layers}          & \textbf{Position}  &                             &                           \\ \midrule
\multirow{2}{*}{Single-hop} & Shallow                  & Subject Last                  & \multirow{5}{*}{×}          & \multirow{5}{*}{×}       & \multirow{5}{*}{×} & 11.70                        & 94.62                     \\ \cline{2-3}
                            & Deeper  & \rule{0pt}{2.5ex}Last                          &                             &                          &                    & 12.10                           & 97.68                          \\ \cline{1-3}
\multirow{3}{*}{Sup}        & Shallow                  & \rule{0pt}{2.5ex}Last                  &           &       &  & 10.00                        & 40.45                     \\ \cline{2-3}
                            & \multirow{2}{*}{Deeper}  & \rule{0pt}{2.5ex}Subject Last                  &                             &                          &                    & 9.03                        & 13.64                     \\
                            &                          & Last                          &                             &                          &                    & \underline{15.50}                       & 54.15                     \\ \midrule
\multirow{6}{*}{Single-hop} & \multirow{6}{*}{Shallow} & \multirow{6}{*}{Subject Last} & \multirow{2}{*}{Single-hop} & \multirow{2}{*}{Deeper}  & Subject Last       & 11.85                       & 95.21                     \\
                            &                          &                               &                             &                          & Last               & 11.33                       & 98.90                      \\ \cline{4-6}
                            &                          &                               & \multirow{4}{*}{Sup}        & \multirow{2}{*}{Shallow} & \rule{0pt}{2.5ex}Subject Last       & 13.97                       & 92.41                     \\
                            &                          &                               &                             &                          & Last               & 12.33                       & 93.45                     \\ \cline{5-6}
                            &                          &                               &                             & \multirow{2}{*}{Deeper}  &\rule{0pt}{2.5ex} Subject Last       & 12.90                        & 94.69                     \\
                            &                          &                               &                             &                          & Last               & \textbf{17.40}                        & 94.74                     \\ 
\bottomrule
\end{tabular}
}
\caption{Comparison of different methods across batch sizes, hop numbers, and edit instances.}
    \label{tab:main_ablation}
\end{table*}

==> ICLR_text/results/main_result.tex <==
% 设置表格内字体命令
\newcommand{\bftab}{\fontseries{b}\selectfont}  % 加粗命令
\vspace{-2mm}
\begin{table}[htbp]
    \centering
    \resizebox{0.9\textwidth}{!}{  % 调整表格宽度到页面宽度，高度自适应
    \renewcommand{\arraystretch}{1.5}  % 设置行间距
    \begin{tabular}{l l c c c}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Batch\_size=1} & \textbf{Batch\_size=1000} & \textbf{Batch\_size=3000} \\
        \midrule
                
        \multirow{8}{*}{GPT-J-6B} & {Base} & 39.63 & - & - \\
        \cmidrule(lr){2-5} 
                                        & {MeLLo$^\diamond$} ~\cite{MQUAKE} & 20.3 & 11.0 & 10.2 \\
         \cmidrule(lr){2-5}  % 在MEND和IKE之间插入横线
                                        & {ROME$^\spadesuit$} ~\cite{ROME} & 7.6 & - & - \\
                                        & {MEMIT$^\spadesuit$}~\cite{MEMIT} & 12.3 & 8.1 & 1.8 \\
                                        & {MEND$^\spadesuit$} ~\cite{MEND} & 11.5 & 4.3 & 3.5\\
                                        & {PMET$^\spadesuit$} ~\cite{pmet} & 11.17 & 11.13 & 11.7 \\
                                        & \textbf{IFMET (ours)} & \bftab{23.04} & \bftab{18.8} & \bftab{17.4} \\
        \bottomrule
    \end{tabular}
    }
    \caption{ \rebuttal{Multi-hop accuracy comparison of different methods on the MQuAKE-3K dataset in a few-shot setting, showing the \textbf{Base} model's performance on the unedited answer and the edited model's performance on the edited answer.} Methods with $^\spadesuit$ indicate weight-modifying methods, while methods with $^\diamond$ are weight-preserving methods. `-' indicates no relevant result, as ROME does not support multiple edits. \rebuttal{\textbf{Note:} the \textbf{Base} model's performance on the edited answer is 7.70 .}} 
    \vspace{-15pt}
    \label{tab:main_result}
\end{table}
% \vspace{-2mm}

==> ICLR_text/results/original_result.tex <==
% 设置表格内字体命令


\newcommand{\cellgray}{\cellcolor[gray]{0.9}}   % 定义浅灰色背景
\newcommand{\good}[1]{\textbf{#1}}        % 方便表示加粗文本
\begin{table}[!ht]
    \centering
    \resizebox{0.95\textwidth}{!}{ 
    \renewcommand{\arraystretch}{1.2}  % 调整行间距
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{|l|c|c c c|c|c c c|}  % 创建表格布局，调整列格式
        \toprule
        \multirow{2}{*}{\textbf{Editor}} & \multicolumn{4}{c|}{\textbf{Edited Answer $\uparrow$}} & \multicolumn{4}{c|}{\textbf{Unedited Answer $\downarrow$}} \\ 
        \cmidrule(lr){2-5} \cmidrule(lr){6-9}
        & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} \\
        \midrule

        
        GPT-J       & 7.70 & 6.03 &16.92&7.00&39.63&38.43&35.9&44.27 \\ 
        GPT-J+{CoT}       & 6.83 & 5.92 &9.23&7.76&42.83&41.56&39.74&47.33 \\ \cmidrule(lr){2-9}
        PMET        &11.17& 12.13 & 16.09 &6.52&29.95&23.60&35.66&41.85 \\ 
        PMET+{CoT}  & 17.04 & 19.84 &14.32&11.91&29.35&23.12&\good{30.43}&43.22 \\ 
        IFMET       &23.04& 20.24 & 15.28 &33.38&23.08&20.18&34.32&\good{24.25} \\
        \cellgray \textbf{IFMET+{CoT}} & \cellgray \good{31.01} & \cellgray \good{31.69} & \cellgray \good{19.49} & \cellgray \good{35.15} & \cellgray \good{21.62} & \cellgray \good{17.71} & \cellgray 30.51 & \cellgray 26.27 \\
        \bottomrule
    \end{tabular}
    }
    }
    \caption{\rebuttal{Multi-hop accuracy} comparison between unedited and edited answers using PMET and our editors \rebuttal{on the MQuAKE-3K dataset}, with edit\_batch = 1. The type of edited fact—Pre, Mid, or Post—depends on the edited data position within the multi-hop reasoning chain. Average accuracy is calculated as the weighted average of results from these three categories, which have respective quantities of 1824, 390, and 786. Additionally,  +CoT denoted the performance incorporating a Chain-of-thought (CoT) prompt. }
    % \vspace{-0.2in}
    \vspace{-10pt}
    \label{tab:position_result}
\end{table}
\vspace{-0.1in}


==> ICLR_text/results/single_ablation_gptj.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{ 
  \centering
     \begin{tabular}{lcllllll}
    \toprule
        \multicolumn{1}{c}{\textbf{Edits}}&\multicolumn{1}{c}{\textbf{Editor}} & \multicolumn{1}{c}{\textbf{Multi-hop} }& \multicolumn{1}{c}{\textbf{Efficacy} } &  \multicolumn{1}{c}{\textbf{Specificity} }  &  \multicolumn{1}{c}{\textbf{Paraphrase} } \\
        \midrule
% &Base & &72.60& 69.47 & 72.70 \\ \midrule
\multirow{7}{*}{1}
&IFMET & {28.38} \goodmetric{($\uparrow$78.0\%)} &{99.56} ($\uparrow$12.8\%)  & {{65.06} ($\downarrow$17.2\%)} & {{90.17} \goodmetric{($\uparrow$5.3\%)}}   \\
&\makecell{w/o $First$} & {23.14} ($\uparrow$45.1\%) & {66.59} \badmetric{($\downarrow$24.6\%)} & {{59.54} \badmetric{($\downarrow$24.3\%)} } & {41.48} \badmetric{($\downarrow$51.6\%)}\\
&\makecell{w/o $Sup$} & {17.69} ($\uparrow$10.9\%) & {100.00} \goodmetric{($\uparrow$13.3\%)} & {{77.71} ($\downarrow$1.2\%) } & {86.24} ($\uparrow$0.7\%) \\
&\makecell{w/o $Last$} & {18.12} ($\uparrow$13.6\%) & {88.21} ($\uparrow$0.0\%) & {{78.60} \goodmetric{($\downarrow$0.0\%)} } & {86.24} ($\uparrow$0.7\%) \\ 
&\makecell{w/o $Deeper$} & {15.07} \badmetric{($\downarrow$5.4\%)} & {99.56} ($\uparrow$12.8\%) & {{70.31} ($\downarrow$10.6\%) } & {86.90} ($\uparrow$1.5\%)\\ %60
&PMET & {{15.94}} &{{88.21}}  & {78.60} & 85.59\\ \midrule % 62
\multirow{7}{*}{100}

&IFMET & {27.07} \goodmetric{($\uparrow$64.8\%)} & {96.29} ($\uparrow$8.1\%) & {69.89} ($\downarrow$9.4\%) & {84.28} \goodmetric{($\uparrow$3.8\%)}  \\
&\makecell{w/o $First$} & {22.71} ($\uparrow$35.1\%) & {73.36} \badmetric{($\downarrow$17.8\%)} & {{69.21} \badmetric{($\downarrow$10.2\%)} } & {{34.72} \badmetric{($\downarrow$57.3\%)} }   \\
&\makecell{w/o $Sup$} & {17.25} ($\uparrow$2.6\%) & {99.13} ($\uparrow$11.3\%) & {{76.63} \goodmetric{($\uparrow$0.6\%)} } & {{84.06} 
 ($\uparrow$3.5\%)}  \\
&\makecell{w/o $Last$} & {15.94} \badmetric{($\downarrow$5.2\%)} & {89.08} ($\downarrow$0.0\%) & {{76.85} ($\uparrow$0.3\%) } & {{81.55} 
 ($\uparrow$0.4\%)}  \\ 
&\makecell{w/o $Deeper$} & {16.16} ($\downarrow$3.9\%) & {99.56} \goodmetric{($\uparrow$11.8\%)} & {{74.67} ($\downarrow$3.2\%) } & {81.00 ($\downarrow$0.3\%)}\\ 
&PMET & {{16.81}} &{{89.08}}  & {{77.07}} & {{81.22}} \\ 
% &PMET & {{16.81} ($\downarrow$38.0\%)} &{{89.08} ($\downarrow$7.5\%) }  & {{77.07} ($\uparrow$10.2\%)} & {{81.22} ($\downarrow$3.7\%)} \\ 
    \bottomrule
    \end{tabular}
    }
 \caption{The results of the ablation experiments on GPT-J-6B model using a subset of MQuAKE-CF. Both the percentages of decrease($\downarrow$) and increase($\uparrow$) are calculated relative to \textbf{PMET} as the baseline. The most significant performance decline is highlighted in \badmetric{red} and the most significant performance increase is highlighted in \goodmetric{green}.}
 \label{tab:ablation_other_gptj}
 \end{table*}

==> ICLR_text/results/single_ablation_llama.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{ 
  \centering
     \begin{tabular}{lcllllll}
    \toprule
        \multicolumn{1}{c}{\textbf{Edits}}&\multicolumn{1}{c}{\textbf{Editor}} & \multicolumn{1}{c}{\textbf{Multi-hop} }& \multicolumn{1}{c}{\textbf{Efficacy} } &  \multicolumn{1}{c}{\textbf{Specificity} } &  \multicolumn{1}{c}{\textbf{Paraphrase} }\\
        \midrule
% &LLaMA-2-7B & & 84.93 & 74.07 & 76.71 \\ \midrule
\multirow{7}{*}{1}
&IFMET & {28.38} \goodmetric{($\uparrow$73.3\%)}&{99.78} \goodmetric{($\uparrow$13.7\%)}  & {{65.50} ($\downarrow$10.8\%)} & {{75.00} \goodmetric{($\uparrow$23.1\%)} } \\
&\makecell{w/o $First$} & {25.76} ($\uparrow$57.3\%) & {56.55} \badmetric{($\downarrow$35.6\%)} & {{62.18} \badmetric{($\downarrow$15.3\%)} } & {{39.08} \badmetric{($\downarrow$35.9\%)} }   \\
&\makecell{w/o $Sup$} & {19.43} ($\uparrow$18.6\%) & {98.68} ($\uparrow$12.4\%) & {70.35 ($\downarrow$4.2\%) } & {{69.00}  
 ($\uparrow$13.2\%)}   \\
&\makecell{w/o $Last$} & {15.72} ($\downarrow$4.1\%) & {88.86} ($\uparrow$1.2\%) & {73.03 \goodmetric{($\downarrow$0.6\%)} }  &{{61.90} ($\uparrow$1.6\%)} \\ 
&\makecell{w/o $Deeper$} & {15.28} \badmetric{($\downarrow$6.8\%)} & {96.72} ($\uparrow$10.1\%) & {{65.61} ($\downarrow$10.7\%) } & {{66.99} ($\uparrow$9.9\%) } \\ 
&\makecell{w $Sup_{model}$} & {26.86} ($\uparrow$64.0\%) & {96.07} ($\uparrow$9.4\%) & {{63.32} ($\downarrow$13.8\%) } & {74.24} ($\uparrow$21.8\%)  \\ 
&PMET & {{16.38}} &{{87.77}}  & {73.41} & {60.92}\\ \midrule
% &PMET & {{16.38} ($\downarrow$43.3\%)} &{{87.77} ($\downarrow$12.1\%) }  & {73.41} ($\uparrow$12.1\%) & {60.92} ($\downarrow$19.8\%) \\ \midrule
\multirow{7}{*}{100}
&IFMET & {27.29} \goodmetric{($\uparrow$76.0\%)}& {97.82} ($\uparrow$4.2\%)  & {{65.50} ($\downarrow$9.9\%)}  & {{84.17} \goodmetric{($\uparrow$14.2\%)}}   \\
&\makecell{w/o $First$} & {24.67} ($\uparrow$59.2\%) & {64.41} \badmetric{($\downarrow$31.4\%)} & {{63.97} ($\downarrow$12.0\%) } & {{41.81} \badmetric{($\downarrow$43.3\%)}  }   \\
&\makecell{w/o $Sup$} & {15.07} ($\downarrow$2.8\%) & {99.34} \goodmetric{($\uparrow$5.8\%)} & {{71.83} ($\downarrow$1.2\%)  }  & {76.64} ($\uparrow$4.0\%) \\
&\makecell{w/o $Last$} & {13.97} \badmetric{($\downarrow$9.9\%)} & {94.32} ($\uparrow$0.4\%) & {{72.14} \goodmetric{($\downarrow$0.8\%)}  } & {{74.67} ($\uparrow$1.3\%) }   \\ 
&\makecell{w/o $Deeper$} & {15.94} ($\uparrow$2.8\%) & {96.51} ($\uparrow$2.8\%) & {{69.48} ($\downarrow$4.4\%)  } & {{75.44} ($\uparrow$2.3\%) } \\ 
&\makecell{w $Sup_{model}$} & {22.49} ($\uparrow$45.1\%) & {96.07} ($\uparrow$2.3\%) & {{63.32} \badmetric{($\downarrow$12.9\%)} } & {79.26} ($\uparrow$7.5\%) \\
&PMET & {{15.50}} &{{93.89}}  & {{72.66}} & {{73.69}}  \\
% &PMET & {{15.50} ($\downarrow$43.2\%)} &{{93.89} ($\downarrow$4.1\%)}  & {{72.66} ($\uparrow$10.9\%)} & {{73.69} ($\downarrow$12.5\%)}  \\
    \bottomrule
    \end{tabular}
    }
 \caption{The results of the ablation experiments on LLaMA-2-7B model using a subset of MQuAKE-CF. \textbf{w $Sup_{model}$} represents the $Sup$ queries generated by model itself to modify deeper MLPs. Both the percentages of decrease($\downarrow$ ) and increase($\uparrow$) are calculated relative to \textbf{IFMET} as the baseline.}
 \label{tab:llama_ablation}
 \end{table*}

==> ICLR_text/table/cot-prompt.tex <==
\begin{table*}[ht]
    \centering
    \small
    \noindent\fbox{%
    \begin{minipage}{1\columnwidth} 
\tt 
Question: What is the capital of the country where Plainfield Town Hall is located?\\
Thoughts: Plainfield Town Hall is located in the country of the United States of America. The capital of United States is Washington, D.C.\\
Answer: Washington, D.C.\\
\\
Question: In which country is the company that created Nissan 200SX located?\\
Thoughts: Nissan 200SX was created by Nissan. Nissan is located in the country of Japan.\\
Answer: Japan\\
\\
\textcolor{gray}{$[$3 in-context demonstrations abbreviated$]$} \\
\\
Question: Who has ownership of the developer of the Chevrolet Corvette (C4)?\\
Thoughts: The developer of Chevrolet Corvette (C4) is Chevrolet. Chevrolet is owned by General Motors.\\
Answer: \textbf{\underline{Model Generated Answer Goes Here}}
    \end{minipage}
}
    \caption{The template of the prompt we used for asking multi-hop questions using chain-of-thoughts.}
    \label{tab:cot_template}
\end{table*}


\begin{table*}[ht]
    \centering
    \small
    \noindent\fbox{%
    \begin{minipage}{1.0\columnwidth} 
\tt 
{\scriptsize
 \textcolor{gray}{\texttt{(In-context-learning examples)}}}\newline
Q: Who is the developer of Telegram? A: Telegram FZ-LLC\newline 
Q: Who is the developer of Microsoft Windows? A: Microsoft\newline 
Q: Who is the developer of PlayStation 2? A: Sony Interactive Entertainment\newline 
Q: Who is the developer of iTunes? A: Apple Inc.\newline 
Q: Who is the developer of SR-71 Blackbird? A: Kelly Johnson\newline 
Q: Who is the developer of Moblin? A: Linux Foundation\newline 
Q: Who is the developer of Xbox 360? A: Microsoft\newline 
Q: Who is the developer of Kinsey scale? A: Alfred Kinsey \newline
{\scriptsize \textcolor{gray}{\texttt{(Query during inference)}}}\newline
Q: Who is the developer of SteamOS? A:Valve Corporation
\end{minipage}
}

    \caption{An example of the prompt we used to recall single-hop fact}
    \label{tab:recall_single_hop}
\end{table*}

\begin{table*}[ht]
    \centering
    \small
    \noindent\fbox{%
    \begin{minipage}{1.0\columnwidth} 
\tt 
{\scriptsize
 \textcolor{gray}{\texttt{(In-context-learning examples)}}}\newline
Q: What is the country where The Rotunda is located? A: United States of America \\
Q: In which country was Tohar Butbul granted citizenship? A: Israel \\
Q: Who was Nissan 200SX created by? A: Nissan\\
Q: What continent is the country where Prickly Pear grows located in? A: Europe\\
Q: What is the capital of the country where Plainfield Town Hall is located? A: Washington, D.C.\\
Q: In which country is the company that created Nissan 200SX located? A: Japan\\
Q: Who was Dodge Ram SRT-10 created by? Dodge\\
Q: Who is the spouse of Joe Biden? A: Jill Biden\\
Q: Which continent is the country where the director of "My House Husband: Ikaw Na!" was educated located in? A: Asia\\
Q: What country was the location of the Battle of Pressburg? A: Hungary\\
Q: Who is the spouse of the US president? A: Jill Biden\\
Q: Who has ownership of the developer of the Chevrolet Corvette (C4)? A: General Motors\\
Q: Who is Joe Biden married to? A: Jill Biden\\
Q: What is the country of citizenship of Charles II of Spain? A: Spain\\
Q: Who was Chevrolet Biscayne created by? A: Chevrolet\\
Q: What is the name of the current head of state in United Kingdom? A: Elizabeth II\\
Q: \textcolor{gray}{multi-hop question}
\end{minipage}
}
    \caption{The template of the prompt we used for asking multi-hop questions using few shot.}
    \label{tab:few-shot-template}
\end{table*}


\begin{table*}[ht]
    \centering
    \small
    \noindent\fbox{%
    \begin{minipage}{1.0\columnwidth} 
\tt 
{\scriptsize
 \textcolor{gray}{\texttt{(In-context-learning examples)}}}\newline
Input: The country that has nationals <mask> is located in the continent of Asia\\
Output: Hitomi Yaida

Input: The country that has nationals <mask> has the official language of Italian\\
Output: Giorgio Chiellini

Input: The university where <mask> was educated located its headquarters in the city of Vienna\\
Output: Michael Haneke

Input: The country that has nationals <mask>, its capital is Washington\\
Output: Lou Pearlman

Input: The person who found <mask> is a citizen of United States of America\\
Outout: Microsoft

Input: The creator of <mask> hails from Italy\\
Output: Ferrari

Input: The author of <mask> is a citizen of United States of America\\
Output: Holly Potter

Input: The person who discovered <mask> lives in Germany\\
Output: Volkswagen\\
Input: \textcolor{gray}{question}
\end{minipage}
}
    \caption{The template of the prompt we used for asking LLaMA-2-7B to generate the supplementary set.}
    \label{tab:model_generate}
\end{table*}

==> ICLR_text/table/method_difference.tex <==
\begin{table*}[t]
\centering
\resizebox{0.8\textwidth}{!}{ 
  \centering
     \begin{tabular}{ccccc}
     \toprule
     \multicolumn{1}{c}{\textbf{Method}}&\multicolumn{1}{c}{\textbf{Stage}} & \multicolumn{1}{c}{\textbf{Data} }& \multicolumn{1}{c}{\textbf{Position} } &  \multicolumn{1}{c}{\textbf{Layers} }  \\ \midrule
Previous             & Only one                                                    & Single-hop                                               & Subject Last Token                                                      & Shallow              \\ \midrule
IFMET                & \begin{tabular}[c]{@{}c@{}}First\\ Furtherance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Single-hop\\ Two-hop($Sup$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Subject Last Token\\ Last Token\end{tabular} & \begin{tabular}[c]{@{}c@{}}Shallow\\ Deeper\end{tabular}        \\
 \bottomrule
\end{tabular}
    }
 \caption{The main difference between \textbf{IFMET} and previous methods. The term \textbf{Stage} refers to the phases of the editing process, \textbf{Data} denotes the query utilized for editing, \textbf{Position} specifies the token position where the editing is applied, and \textbf{Layers} indicate the edited layers.
}
 \label{method_difference}
 \end{table*}

==> ICLR_text/table/sparql.tex <==
\begin{table*}[ht]
    \centering
    \small
    \noindent\fbox{%
    \begin{minipage}{0.8\columnwidth} 
\tt 
SELECT ?subject ?subjectLabel ?predicate ?predicateLabel WHERE {{ \\
      ?subject ?predicate wd:{ss}.  \\
      FILTER (?predicate IN (wdt:{relation}))  \\
      SERVICE wikibase:label {{ bd:serviceParam wikibase:language "en". }} \\
    }}
 LIMIT 50
    \end{minipage}
}
    \caption{The template of the SPARQL Query we used for the supplementary triplets.}
    \label{tab:sparql_template}
\end{table*}

==> ICLR_text/table/time_table.tex <==
\begin{table*}[t]
\centering
\resizebox{0.4\textwidth}{!}{ 
  \centering
     \begin{tabular}{ccccc}
     \toprule
     \multicolumn{1}{c}{\textbf{Model}}&\multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Time} } \\ \midrule
\multirow{3}{*}{GPT-J-6B}     
& MEMIT & 4.5s \\
& PMET  & 5.0s \\
& IFMET & 9.7s \\ \midrule
\multirow{3}{*}{LLaMA-2-7B} 
& MEMIT & 2.1s \\
& PMET  & 2.0s \\
& IFMET & 3.4s \\ \bottomrule
\end{tabular}
    }
 \caption{The average time required to edit a single case varies across methods. For the two one-stage methods, \textbf{MEMIT} and \textbf{PMET}, this corresponds to the process of optimizing the shallow-layer MLPs using single-hop queries. For \textbf{IFMET}, the process includes updating the deeper-layer MLPs using two-hop supplementary sets.
}
 \label{time_difference}
 \end{table*}

==> macro.tex <==

\titlespacing*\section{0pt}{12pt plus 5pt minus 5pt}{9pt plus 3pt minus 3pt}


\hypersetup{
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}


\usepackage{amsmath,amsfonts,bm}
\usepackage{xifthen}
\usepackage{xparse}

\catcode`\_=11\relax
 \newcommand\email[1]{\_email #1\q_nil}
\def\_email#1@#2\q_nil{%
  \href{mailto:#1@#2}{{\emailfont #1\emailampersat #2}}
}
 \newcommand\emailfont{\rmfamily \lsstyle}
 \newcommand\emailampersat{@}
\catcode`\_=8\relax 


\definecolor{ggreen}{rgb}{0.0, 0.6, 0.0}
\definecolor{rred}{rgb}{0.75, 0.0, 0.0}
\definecolor{bblue}{rgb}{0.13, 0.67, 0.8}

 \newcommand{\badmetric}[1]{{\color{rred} \textbf{#1}}}
 \newcommand{\goodmetric}[1]{{\color{ggreen} \textbf{#1}}}
 \newcommand{\mehmetric}[1]{{\color{olive} \textbf{#1}}}


 \newcommand{\yb}[1]{\todo{YB: #1}}
 \newcommand{\reminder}[1]{ (\mbox{$\star$}{\textbf{\textcolor{blue}{#1}}}\mbox{$\star$})}


 \newcommand{\rewg}{G^\prime}  %
 \newcommand{\mlp}{\mathrm{mlp}\xspace}
 \newcommand{\attn}{\mathrm{attn}\xspace}
 \newcommand{\cfd}{\textsc{CounterFact}\xspace}
 \newcommand{\cfdabbr}{\textsc{CF}\xspace}
 \newcommand{\pararel}{\textsc{ParaRel}\xspace}
 \newcommand{\efk}{Knowledge Editor\xspace}
 \newcommand{\dkn}{Knowledge Neurons\xspace}
 \newcommand{\methodlong}{MEMIT\xspace}
 \newcommand{\method}{MEMIT\xspace}
 \newcommand{\neox}{GPT-NeoX\xspace}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}

 \newcommand{\atl}[2]{#1^{#2}}
 \newcommand{\elid}[2]{#1_{#2}}
 \newcommand{\ex}[1]{\mathbb{E}\left[ #1 \right]}
 \newcommand{\exsub}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
 \newcommand{\pr}[1]{\mathbb{P}\left[ #1 \right]}
 \newcommand{\prsub}[2]{\mathbb{P}_{#2}\left[ #1 \right]}
 \newcommand{\indic}[1]{\mathbb{I}\left[ #1 \right]}
 \newcommand{\pprime}{{\prime\prime}}


 \newcommand{\fid}{Fr\'echet Inception Distance\xspace}
 \newcommand{\concepts}{object concepts\xspace}
 \newcommand{\pgan}{Progressive GANs\xspace}
 \newcommand{\featuremap}{featuremap\xspace}
 \newcommand{\mask}{\texttt{mask}}
 \newcommand{\threshold}{\text{T}}
 \newcommand{\pixel}{\text{P}}
 \newcommand{\pixelall}{\sP}
 \newcommand{\KL}{D_{\mathrm{KL}}}
 \newcommand{\context}{K}
 \newcommand{\U}{\text{U}}
 \newcommand{\Uall}{\sU}

 \newcommand{\thresU}{\rvk}
 \newcommand{\thresUall}{\rvk}
 \newcommand{\rUP}{\repr_{\U, \pixel}}
 \newcommand{\rUPb}{\repr_{\overline{\U, \pixel}}}
 \newcommand{\rUb}{\repr_{\overline{\U}, \pixel}}
 \newcommand{\pp}{\repr_{\Uall, \pixel}}
 \newcommand{\ppb}{\repr_{\Uall, \overline{\pixel}}}
 \newcommand{\contextr}{\context^*}
 \newcommand{\Ezp}{\E_{\rvz,\pixel}}
 \newcommand{\IoU}{\text{IoU}}
 \newcommand{\ACE}{\delta}
 \newcommand{\ACEUc}{\ACE_{\U\rightarrow c}}
 \newcommand{\xinsert}{\rvx_{i}}
 \newcommand{\xablate}{\rvx_{a}}
 \newcommand{\layer}[1]{\texttt{layer#1\xspace}}
 \newcommand{\unit}[1]{\texttt{unit#1\xspace}}
 \newcommand{\vA}{\bm{\alpha}}
 \newcommand{\G}{G}
 \newcommand{\seg}{\rvs_c}
 \newcommand{\repr}{\rvr}
 \newcommand{\repru}{\repr_{u, \sP}}
 \newcommand{\uprepru}{\repr_{u, \sP}^{\uparrow}}
 \newcommand{\f}{f}
 \newcommand{\h}{h}

 \newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

 \newcommand{\figleft}{{\em (Left)}}
 \newcommand{\figcenter}{{\em (Center)}}
 \newcommand{\figright}{{\em (Right)}}
 \newcommand{\figtop}{{\em (Top)}}
 \newcommand{\figbottom}{{\em (Bottom)}}
 \newcommand{\captiona}{{\em (a)}}
 \newcommand{\captionb}{{\em (b)}}
 \newcommand{\captionc}{{\em (c)}}
 \newcommand{\captiond}{{\em (d)}}

 \newcommand{\newterm}[1]{{\bf #1}}

 \newcommand{\reffig}[1]{Figure~\ref{fig:#1}}
 \newcommand{\refsec}[1]{Section~\ref{sec:#1}}
 \newcommand{\refapp}[1]{Appendix~\ref{sec:#1}}
 \newcommand{\reftbl}[1]{Table~\ref{tbl:#1}}
 \newcommand{\refalg}[1]{Algorithm~\ref{alg:#1}}
 \newcommand{\refline}[1]{Line~\ref{line:#1}}
 \newcommand{\shortrefsec}[1]{\S~\ref{sec:#1}}
 \newcommand{\refeqn}[1]{Eqn.~\ref{eq:#1}}
 \newcommand{\refeqshort}[1]{(\ref{eq:#1})}
 \newcommand{\shortrefeq}[1]{\ref{eq:#1}}
 \newcommand{\lblfig}[1]{\label{fig:#1}}
 \newcommand{\lblsec}[1]{\label{sec:#1}}
 \newcommand{\lbleq}[1]{\label{eq:#1}}
 \newcommand{\lbltbl}[1]{\label{tbl:#1}}
 \newcommand{\lblalg}[1]{\label{alg:#1}}
 \newcommand{\lblline}[1]{\label{line:#1}}
 \newcommand{\ignorethis}[1]{}
 \newcommand{\revision}[1]{\color{black}#1\color{black}}
 \newcommand{\myitem}{\vspace{-5pt}\item}
 \newcommand{\myparagraph}[1]{\vspace{-5pt}\paragraph{#1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
 \newcommand{\train}{\mathcal{D}}
 \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
 \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
 \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

 \newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

 \newcommand{\pdata}{p_{\rm{data}}}
 \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
 \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
 \newcommand{\pmodel}{p_{\rm{model}}}
 \newcommand{\Pmodel}{P_{\rm{model}}}
 \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
 \newcommand{\pencode}{p_{\rm{encoder}}}
 \newcommand{\pdecode}{p_{\rm{decoder}}}
 \newcommand{\precons}{p_{\rm{reconstruct}}}

 \newcommand{\laplace}{\mathrm{Laplace}} %

 \newcommand{\E}{\mathbb{E}}
 \newcommand{\Ls}{\mathcal{L}}
 \newcommand{\R}{\mathbb{R}}
 \newcommand{\emp}{\tilde{p}}
 \newcommand{\lr}{\alpha}
 \newcommand{\reg}{\lambda}
 \newcommand{\rect}{\mathrm{rectifier}}
 \newcommand{\softmax}{\mathrm{softmax}}
 \newcommand{\sigmoid}{\sigma}
 \newcommand{\softplus}{\zeta}
 \newcommand{\Var}{\mathrm{Var}}
 \newcommand{\standarderror}{\mathrm{SE}}
 \newcommand{\Cov}{\mathrm{Cov}}
 \newcommand{\normlzero}{L^0}
 \newcommand{\normlone}{L^1}
 \newcommand{\normltwo}{L^2}
 \newcommand{\normlp}{L^p}
 \newcommand{\normmax}{L^\infty}

 \newcommand{\parents}{Pa} %

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak



\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

 \newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
 \newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

 \newcommand{\shapenet}{ShapeNet\xspace}
 \newcommand{\pascal}{PASCAL 3D+\xspace}

 \newcommand{\degree}{\ensuremath{^\circ}\xspace}
 \newcommand{\ignore}[1]{}
 \newcommand{\norm}[1]{\lVert#1\rVert}
 \newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand{\thefootnote}{\arabic{footnote}}


\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot,\xspace} 
\def\Eg{E.g\onedot,}
\def\ie{i.e\onedot,\xspace} 
\def\Ie{\emph{I.e}\onedot,}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}
 \newcommand{\iclrnew}[1]{#1}

==> packages.tex <==
\usepackage{color,xcolor}
\usepackage{epsfig}
\usepackage{graphicx}

\usepackage{tikz}
\usetikzlibrary{arrows}

\usepackage{listings}
\usepackage{esdiff}
\usepackage{mdframed}
\newmdenv[
  backgroundcolor=gray!20,
  skipabove=\topsep,
  skipbelow=\topsep,
  roundcorner=2mm
]{gentext}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\usepackage{tabularx}
\usepackage{adjustbox}
\usepackage{array}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{numprint}

\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}
\usepackage{dsfont}

\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{hyperref}       %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %



\usepackage{changepage}
\usepackage{extramarks}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}
\usepackage{lipsum}



\usepackage{algorithm2e}
\usepackage{enumitem}

\usepackage{titlesec}

\usepackage[page]{appendix}
\usepackage[hang,flushmargin]{footmisc}



==> save_writting.tex <==
Specific method introduction

We primarily based our work on the MQUAKE-CF dataset, transforming the edit case into a single-hop dataset for our investigation. To simplify the scenario, we selected only the two-hop fact recall subset from MQUAKE. Additionally, we extended the original dataset by providing a comprehensive range of prompts in different formats based on the relative positions of the subject and relation.

\textbf{Exploration of Knowledge Storage and Reasoning Mechanisms.} By investigating the characteristics of the model's knowledge storage for the subject entity, We found that the model couples the storage of different knowledge related to the same subject and exhibits similar preferences. Knowledge related to a specific relation only decouples from other knowledge when activated by that relation. The language model tends to aggregate knowledge in the earlier to middle layers and further enhance this knowledge in the subsequent layers. This is evidenced by a rank that initially drops to a small value before the probabilities accumulate. But in multi-hop scenarios, we additionally focused on the trends of changes in intermediate reasoning results, which are the entities produced by the first-hop relation. We discovered inconsistent model behavior: the aggregation of final results occurring more slowly and the aggregation of intermediate results occurring less significantly, with a notable reduction in probability accumulation in the later layers.

\textbf{Exploration from a Circuit Perspective.} After discovering the aforementioned inconsistencies in behavior, we attempted to investigate the model structure to identify subgraphs that execute factual recall tasks, which are referred to as \textbf{\emph{'knowledge circuits'}} in previous work. By using the knowledge circuits independently, the language model can achieve or even exceed its original performance in recalling facts, demonstrating the effectiveness of these discovered knowledge circuits. And the circuits exhibit consistent performance across different hop datasets. When comparing the distribution of activated components and edges with the Pearson correlation coefficients, We found that single-hop and multi-hop tasks share structural similarities in their knowledge circuits. The main difference arises from the connections between MLP layers, that is because \highlight{wait to complete}

Additionally, we delved into the information flow of specific knowledge within the circuits, and identified several key components (e.g., attention heads) that play crucial roles in transmitting information to the final token positions and capturing relational information from the context. We discovered that both single-hop and multi-hop factual recall utilize some common attention heads such as \highlight{wait to complete}. There are certain specific mechanisms in multi-hop reasoning, which are \highlight{wait to complete}.

\textbf{Exploration of the Impact of Knowledge Editing.} From the perspective of knowledge storage, we observed that in edited model, the edited knowledge tends to dominate all knowledge associated with the subject. Specifically, under the activation of any relation, the model shows a tendency to output the newly edited knowledge in specific cases. We also explored the flow of information of the edited knowledge within the circuit in single-hop factual recall scenarios, finding that it aligns with the original model's behavior. This indicates that the model has indeed modified the corresponding knowledge in the MLP that contributes information. In multi-hop factual recall scenarios, we discovered that the flow of information for the edited knowledge within the circuit reveals \highlight{wait to complete}, suggesting that \highlight{wait to complete}.

\textbf{Enhancing Existing Editing Methods.} Finally, based on the unified framework of editing methods proposed in previous work, we implemented an interpretable layer propagation method and in light of the mechanisms underlying multi-step factual recall introduced a secondary editing method that alleviates the poor performance of existing locate-then-edit model editing methods in multi-step factual recall scenarios.

In summary, this paper addresses three key questions: First, we explore the underlying mechanisms of the model's multi-hop factual recall from a circuit perspective, highlighting the similarities and differences with single-hop from the viewpoints of active component and reasoning processes. Then, By comparing models edited with existing knowledge editing methods for single-hop facts, we investigate multi-hop questions that the original model could answer but fail to after editing, and assess whether the reasoning process for both single-hop and multi-hop tasks remains consistent with the original model. Finally, We apply these insights within a unified framework to enhance existing editing methods, focusing primarily on two aspects: layer distribution algorithms and secondary editing methods. These improvements not only boost the editing performance of KE methods in traditional single-hop factual recall tasks but also mitigate the poor utilization performance in multi-hop factual recall tasks.
\highlight{Wait to summary the contribution and introduce the following section structure}

==> text/method_orig.tex <==
% \newcommand{\Km}[2]{\left[ k_1^{#1} \, \vert \, k_2^{#1} \, \vert \, \cdots \, \vert \, k_{#2}^{#1} \right]}
% \newcommand{\Vm}[2]{\left[ v_1^{#1} \, \vert \, v_2^{#1} \, \vert \, \cdots \, \vert \, v_{#2}^{#1} \right]}
\section{Enhanced Existing Knowledge Editing \di{CHnage the title}}
% Single case in the knowledge editing task can be simply summarized as following quadruple: \( p(s, r), o, o^*, p_{\text{test}} \), where $p(s,r)$ is the Cloze-Format prompt used for editing the knowledge. $o$ and $o^*$ represent the original and new object, respectively. And \( p_{\text{test}} \) denotes the prompt used to test different type of performance of editing method. It may either be the same or a rephrasing of \( p(s, r) \), or it could involve other subjects sharing the same relation $p(s_r,r)$. And The whole set with multiple knowledge editing cases denoted as 
% $
% \{(p(s_i, r_i), o_i, o_i^*, p_{\text{test},i}) \mid i = 1, 2, \dots, E\},
% $
% where each element follows the same structure. \di{No, this should be included in  preliminaries, not here}


% \subsection{Unified Framework of existing methods} 
% \di{The whole section is about previous method, I think you should move to preliminaries. }
% Following previous work, we adopt a unified framework to explore locate-then-edit methods. We demonstrate that approaches like ROME, MEMIT, PMET, and EMMET are variations of this framework. 

% \noindent {\bf Preserve-Edit Objective } Like \cite{memory_key_value} and \cite{ROME}, we treat the Feed-Forward Network(FFN) as a key-value store for knowledge. Let \( W_0 \) denote the original weights of the FFN that needs modifying. The \( k \), input vector of $W_0$, acting as a lookup \textbf{key}, represents entities of interest $s$ or some specific fact $(s,r)$. The hidden states produced after passing through the FFN are treated as \textbf{values} \( v \), which represent the knowledge associated with \( k \), retrieved from the weights \( W \). And \( v\) is typically considered to contain information about \( o \). So that a \((k,v)\) pairs, satisfying $Wk = v$, represent the full fact $\left( s, r, o \right)$. After Knowledge Editing, the weights of FFN are changed from $W_0$ to $W_e$ , we can define the objective of knowledge preservation and editing:
% \[
% \underbrace{\mathbf{P}(\hat{W},K_0,V_0)}_{\text{Preserve}}
% \quad \text{and} \quad
% \underbrace{\mathbf{E}(\hat{W},K_e,V_e)}_{\text{Edit}}
% \]
% Where $K_0 = \Km{0}{N}$ and $V_0 =  W_0 K_0$ containing all the knowledge we want to preserve in a row. $K_E = \Km{e}{E}$ is a matrix containing the edits we try to make and $V_e = \Vm{e}{E}$ represents the target representations of the new knowledge. ($K_E,V_E$) corresponds to the edited fact set  $\{\left( s_i, r_i, o^*_i \right) \vert i = 1,2,\cdots,E\}$. The differences between these existing methods lie in the selection of the preservation objective $\mathbf{P}$ and the editing objective $\mathbf{E}$. For instance, if we use least squares method to constrain both the preservation and edit, we obtain MEMIT: 
% \[
% \argmin_{\hat{W}} \left( \lambda \underbrace{\| \hat{W} K_0 - W_0 K_0 \|^2}_{\text{Preserve}} + \underbrace{\| \hat{W} K_E - V_E \|^2}_{\text{Edit}} \right)
% \]

% Different types of constraints lead to different optimization methods, but ultimately yield solutions of similar form: $ \hat{W} = W_0 + \Delta$ where $\Delta$ is a function of $W_0, V_E,  K_E$. Specific functions used to compute $\Delta$ and more optimization objectives of other methods refer to the Appendix.

% \noindent {\bf FFN selection and Edit-Layer-Propagation Algorithms } Through causal tracing methods, these method select the second FFN in MLP as the target to edit knowledge. When find the $V_E$, they propagate the desired updates of \textbf{values} vector $R = V_E-W_0K_E$ across all the critical layers. We refer to this algorithm as an \textbf{Edit-Layer-Propagation Algorithms}, applied post-hoc after finding the closed-form solutions to the PE-objective. This has contributed to the outstanding performance of MEMIT and PMET in editing tasks, particularly with large batch sizes. 

% \noindent {\bf  Target value vector of the new knowledge } To obtain the target \textbf{values} vector of the new knowledge $V_E$, these methods use an objective function based on KL divergence and maximizing $\mathbb{P}[o^*|p(s,r)]$, the output probability of the edited knowledge in prediction layer. For further details, please refer to the Appendix.

% \subsection{IDMET method}

% \noindent {\bf Interpretable Edit-Layer-Propagation Algorithm } As we observed in \ref{components}, each individual MLP contributes by \textit{adding} to related knowledge at specific tokens, which is later read by last-token attention modules, and the related knowledge is gradually accumulated over layers. Thus, \cite{MEMIT} propose using the \textbf{Edit-Layer-Propagation Algorithm} to achieve more effective knowledge transfer. Let $A$ represent the weight matrix for propagation between layer $i$ and layer $j$, $A = [f_{ij}]$ with $f_{ij} = g(i, j)$. Compared to MEMIT's use of even distribution $g(i, j)=\frac{1}{j-i+1}$, PMET employs $g(i, j)=\frac{1}{\sqrt{j-i+1}}$ to transmit more precise information to the critical layers. However, these algorithms function more like a hyperparameter and lack interpretability. Given that the circuit's edges model the influence of one component's output on another, they can be effectively applied it to optimize edge propagation algorithms, wthich we called  Interpretable Edit-Layer-Propagation Algorithm(IEPA). \di{Why you are still introducing previous method? }


% \noindent {\bf Furtherance Editing For Multi-hop} 


% \setlength{\algomargin}{10pt}
% \RestyleAlgo{ruled}
% \newlength{\commentWidth}
% \setlength{\commentWidth}{7cm}
% \newcommand{\atcp}[1]{\tcp*[f]{\makebox[\commentWidth]{#1\hfill}}}
% \newcommand{\atcpl}[1]{\tcp*[r]{\makebox[\commentWidth]{#1\hfill}}}
% \newcommand\mycommfont[1]{\footnotesize\textcolor{blue}{#1}}
% \newcommand{\elid}[2]{#1_{#2}}
% \newcommand{\tresid}{\elid{\delta}{i}}
% \newcommand{\prsub}[2]{\mathbb{P}_{#2}\left[ #1 \right]}
% \newcommand{\atl}[2]{#1^{#2}}
% \newcommand{\refeqn}[1]{Eqn.~\ref{eq:#1}}
% \newcommand{\method}{MEMIT\xspace}
% \newcommand{\Gsub}{G(\atl{h}{L}_i\mathrel{+}=\tresid)}
% \SetCommentSty{mycommfont}
% \begin{center}
% % \scalebox{0.9}{
% \begin{minipage}{\linewidth}
% \begin{algorithm}[H]
% \SetAlgoLined
% \caption{The IDMET Algorithm}\label{alg:mrome}
% \KwData{Requested edits $\mathcal{E} = \{ (s_i, r_i, o_i) \}$, generator $G$, layers to edit $\mathcal{S}$, covariances $C^l$}
% \KwResult{Modified generator containing edits from $\mathcal{E}$}

% \For(\quad \atcp{Compute target $z_i$ vectors for every memory $i$}){$s_i, r_i, o_i \in \mathcal{E}$}{
%     \textbf{optimize} $\delta_i \leftarrow \argmin_{\delta_i    } \frac{1}{P} \sum_{j=1}^P -\log\prsub{o_i \mid x_j \oplus p(s_i, r_i)}{\Gsub}$ (\refeqn{compute-z}) \;
%     $z_i \gets \atl{h}{L}_i + \delta_i$ \;
% }
% \For(\quad \atcp{Perform update: spread changes over layers}){$l \in \mathcal{R}$}{
%     $\atl{h}{l}_i \gets \atl{h}{l-1}_i + \atl{a}{l}_i + \atl{m}{l}_i$ (\refeqn{autoregressive}) \quad \atcpl{Run layer $l$ with updated weights}
    
%     \For{$s_i, r_i, o_i \in \mathcal{E}$}{
%         $k^l_i \gets \atl{k}{l}_i = \frac{1}{P} \sum_{j=1}^P k(x_j + s_i)$ (\refeqn{compute-k}) \;
%         $r^l_i \gets \frac{z_i - \atl{h}{L}_i}{L - l + 1}$ (\refeqn{compute-v}) \quad \atcpl{Distribute residual over remaining layers}
%     }
%     $K^l \gets$ \texttt{[$k^{l_1}_i, ... ,k^{L}_i$]}  \quad \atcpl{Update }
%     $R^l \gets$ \texttt{[$r^{l_1}_i, ... ,r^{L}_i$]} \;
%     $\Delta^l \gets R^l {K^l}^T (C^l + K^l {K^l}^T)^{-1}$ (\refeqn{multirome-update})   \;
%     $W^l \gets W^l + \Delta^l$ \quad \atcpl{Update layer $l$ MLP weights in model}
% }
% \end{algorithm}%
% \end{minipage}%
% % }%
% \end{center}



==> text/rebuttal.tex <==
\noindent {\bf Official Review of Submission3638 by Reviewer Pi7C}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item For Q1, We have widened Figures 2(a) and 2(b) and enlarged the subfigures in Figure 7(Figure 6 in previous version) to improve visibility.
    \item For weakness 1,2 and Q2, We revised the terminology in Tables and Figures, to consistently refer to the unmodified model as "Base". Additionally, we included a unified explanation of this term in the \textbf{Baseline} section of \textbf{5.1 Experimental Setup}. Then We provided detailed explanations of the reported outcomes in tables in the \textbf{Setup and Hyperparameters section} of \textbf{5.1 Experimental Setup}, ensuring consistent definitions for \textbf{"original answer"} and \textbf{"edited answer".} Notes have also been added below each table to clarify the meaning of these values. We hope this explaination address your concerns about Questionable Analysis of Results in Table 3 and others.
    \item For weakness 3 To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. Importantly, they confirm that the observed performance improvements are not solely attributable to the supplementary set.
\end{enumerate}
Regarding the organization of the paper, we fully understand the difficulties you encountered when important results were placed in the appendix. We spent considerable time attempting to incorporate more tables into the main text but were ultimately unsuccessful. At the same time, we believe that the analytical section preceding the experiments is necessary. Therefore, we kindly ask for your understanding that due to space constraints, we had to place some tables, and even the entire ablation study, in the appendix. Our aim was to preserve the completeness of the experimental results as much as possible. All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer 1m6u}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item We have corrected the typo errors you mentioned(Line 387, cizizenship $\rightarrow$ citizenship, Figure 1, Mardrid $\rightarrow$ Madrid.) and The biblology style has been consistent.
    \item Ablation study Analyses: To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position.
    \item For weakness 1, we first extended the causal intervention experiments to the LLaMA2-7B model, demonstrating the consistency of interpretability analysis while validating the effectiveness of our method. You can check it in Figure 6 and Table 9 in new version.
    \item For wakness 2: We constructed the paraphrase set and neighborhood set for a subset of the MQuAKE-CF dataset, following the approach used in the COUNTERFACT dataset. The results indicate that IFMET outperforms single-stage editing methods (PMET) in Multi-hop Accuracy, Efficacy Score, and Paraphrase Score, with only a minor decrease in the Neighborhood Score. For more details on related ablation studies, please refer to the corresponding section.
    \item For weakness 3: We compared the time complexity of \textbf{IFMET} with that of the one-stage \textbf{PMET} method it builds upon. On average,the time required to perform a complete edit for a single case on GPT-J using \textbf{IFMET} was approximately 2.5$\times$ that of \textbf{PMET}. For LLaMA-2, the time required was about 1.5$\times$ that of \textbf{PMET}. We believe this is within an acceptable range, and as the editing speed of the single-stage method improves, the \textbf{IFMET} framework will correspondingly become faster.
    \item For weakness 4: we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Construction of the supplementary set}, providing a detailed explanation on utilizing the model itself to generate the supplementary set.
    \item The application of IFMET to unstructured knowledge editing presents a compelling avenue for further research. Unstructured text inherently encompasses more complex semantic information, and in scenarios involving longer and more intricate texts, the presence of noise can significantly complicate the reasoning process. At present, combining \textbf{IFMET} with efficient fact triple extraction techniques appears to be a feasible approach. We believe this context warrants deeper investigation in future work.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer bAUb}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item Ablation study and Generalizability Analyses: To prove that editing the deeper layers specifically contributes to performance improvement. We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. And we discuss the generalizability of our method in many perspectives
    \item For discussion on why IFMET is superior to these RAG-based methods: we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Comparison with Weight-Preserving Methods}, providing a detailed explanation on why we try to explore the potential of locate-then-edit approach.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.

\noindent {\bf Official Review of Submission3638 by Reviewer ocTZ}

A: Thank you for your positive feedback on our paper and for your valuable suggestions. In response:
\begin{enumerate}
    \item The index of figures and tables are updated. Figure 6 $\rightarrow$ Figure 7, Table 5 $\rightarrow$ 11, Table 6 $\rightarrow$ 10.
    \item For weakness 1, we add a subsection in the appendix section \textbf{E.2 GENERALIZABILITY OF IFMET} called \textbf{Construction of the supplementary set}, providing a detailed explanation on utilizing the model itself to generate the supplementary set.
    \item For weakness 2, We have added a comprehensive ablation study and generalizability analysis in the appendix section \textbf{E ABLATION STUDY AND GENERALIZABILITY OF IFMET}. These results demonstrate the positive contributions of the supplementary set and the interpretability-guided targeting of later MLP layers and the last token position. And we discuss the generalizability of our method in many perspectives
    \item For weakness 3, We revised the terminology in Tables and Figures, to consistently refer to the unmodified model as "Base". Additionally, we included a unified explanation of this term in the \textbf{Baseline} section of \textbf{5.1 Experimental Setup}. Then We provided detailed explanations of the reported outcomes in tables in the \textbf{Setup and Hyperparameters section} of \textbf{5.1 Experimental Setup}, ensuring consistent definitions for \textbf{"original answer"} and \textbf{"edited answer".} Notes have also been added below each table to clarify the meaning of these values. We hope this explaination address your concerns about Questionable Analysis of Results in Table 3 and others.
\end{enumerate}
All changes are highlighted in blue in the revised PDF file. We hope these revisions address your concerns comprehensively.
Regarding the organization of the paper, we fully understand the difficulties you encountered when important results were placed in the appendix. We spent considerable time attempting to incorporate more tables into the main text but were ultimately unsuccessful. At the same time, we believe that the analytical section preceding the experiments is necessary. Therefore, we kindly ask for your understanding that due to space constraints, we had to place some tables, and even the entire ablation study, in the appendix. Our aim was to preserve the completeness of the experimental results as much as possible.


==> text/results/ablation_3000.tex <==
\begin{table*}[t]
\centering
\resizebox{0.65\textwidth}{!}{ 
  \centering
     \begin{tabular}{lcllllll}
    \toprule
        \multicolumn{1}{c}{\textbf{Edits}}&\multicolumn{1}{c}{\textbf{Editor}} & \multicolumn{1}{c}{\textbf{Multi-hop Acc} }& \multicolumn{1}{c}{\textbf{Efficacy} } \\
        \midrule
\multirow{6}{*}{3000}
&IFMET & {\textbf{17.40} \goodmetric{($\uparrow$48.7\%)}} &{94.74} ($\uparrow$0.1\%)  \\
&\makecell{w/o $First$} & {15.50} ($\uparrow$32.4\%) & {54.15} (\badmetric{$\downarrow$42.8\%})  \\
&\makecell{w/o $Sup$} & {11.33} (\badmetric{$\downarrow$3.2\%}) & {98.90} \goodmetric{($\uparrow$4.5\%)}  \\
&\makecell{w/o $Last$} & {12.90} ($\uparrow$10.2\%) & {94.69} ($\downarrow$0.1\%) \\ 
&\makecell{w/o $Deeper$} & {12.33} ($\uparrow$5.3\%) & {93.45} ($\downarrow$1.2\%) \\
&PMET & {{11.70}} &{{94.62}} \\ 
% &PMET & {{11.70} ($\downarrow$32.8\%)} &{{94.62} ($\downarrow$0.1\%)} \\ 
    \bottomrule
    \end{tabular}
    }
 \caption{The results of the ablation experiments of MQuAKE-3K on GPT-J-6B model. \textbf{w/o $First$} represents only optimizing the deeper MLPs with $Sup$ without modifying shallow MLPs first. 
 \textbf{w/o $Sup$} represents reusing Single-hop rewrite query used in first stage rather than the $Sup$ queries to modify deeper MLPs. \textbf{w/o $Last$} represents second stage editing occured in subject last token position.  \textbf{w/o $Deeper$} represents apply second stage editing in shallow MLPs. \textbf{PMET} represents the original one-stage method we used. Both the percentages of decrease($\downarrow$) and increase($\uparrow$) are calculated relative to \textbf{PMET} as the baseline. The most significant performance decline is highlighted in \badmetric{red} and the most significant performance increase is highlighted in \goodmetric{green}.
}
 \label{tab:ablation_3000}
 \end{table*}

==> text/results/hop_num_table.tex <==
% 设置表格内字体命令

\begin{table}[htbp]
    \centering
    \resizebox{0.8\textwidth}{!}
    {  % 调整表格宽度到页面宽度，高度自适应
    \renewcommand{\arraystretch}{1.2}  % 设置行间距
    \begin{tabular}{l l c c c c}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Average Accuracy} & \textbf{2-hop} & \textbf{3-hop} & \textbf{4-hop} \\
        \midrule
                
        \multirow{8}{*}{GPT-J-6B} & {Base} & 42.83 & 48.9 &30.7& 48.9\\
         \cmidrule(lr){2-6}  % 在MEND和IKE之间插入横线
                                        & {FT} & 1.9 & 3.7 & 1.4 & 0.5 \\
                                        & {MEND} & 11.5 & 13.9 & 11.3& 9.5 \\
                                        & {ROME}  & 18.1 & 33.8 & 9.1& 11.4\\
                                        & {MEMIT}  & 12.3 & 22.5 & 6.0& 8.4 \\
                                        & {PMET}  & 17.04 & 26.65 & 12.76&11.7\\
                                        & \textbf{IFMET (ours)} & \bftab{31.01} & \bftab{44.06} & \bftab{23.58} & \bftab{25.4}\\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Multi-hop Acc} Performance comparing the baseline and our method with CoT on multi-hop questions in MQuAKE-3k, categorized by hop counts of {2, 3, 4}. \textbf{Base} in this table represents unmodified GPT-J-6B model, and we report its performance on \textbf{unedited answer} with CoT.}
    \label{tab:hop_result}
\end{table}



==> text/results/main_ablation.tex <==
% 设置表格内字体命令


% \newcommand{\cellgray}{\cellcolor[gray]{0.9}}   % 定义浅灰色背景
% \newcommand{\good}[1]{\textbf{#1}}        % 方便表示加粗文本
% \begin{table}[!ht]
%     \centering
%     \renewcommand{\arraystretch}{1.2}  % 调整行间距
%     \resizebox{\textwidth}{!}{ 
%     \begin{tabular}{|l|c|c c c|c|c c c|}  % 创建表格布局，调整列格式
%         \toprule
%         \multirow{2}{*}{\textbf{Editor}} & \multicolumn{4}{c|}{\textbf{Correct Answer $\uparrow$}} & \multicolumn{4}{c|}{\textbf{Original Answer $\downarrow$}} \\ 
%         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%         & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} & \textbf{Average Accuracy} & \textbf{Pre} & \textbf{Mid} & \textbf{Post} \\
%         \midrule

        
%         GPT-J       & 7.70 & 6.03 &16.92&7.00&39.63&38.43&35.9&44.27 \\ 
%         GPT-J+{CoT}       & 6.83 & 5.92 &9.23&7.76&42.83&41.56&39.74&47.33 \\ \cmidrule(lr){2-9}
%         PMET        &11.17& 12.13 & 16.09 &6.52&29.95&23.60&35.66&41.85 \\ 
%         PMET+{CoT}  & 17.04 & 19.84 &14.32&11.91&29.35&23.12&\good{30.43}&43.22 \\ 
%         IFMET       &23.04& 20.24 & 15.28 &33.38&23.08&20.18&34.32&\good{24.25} \\
%         \cellgray \textbf{IFMET+{CoT}} & \cellgray \good{31.01} & \cellgray \good{31.69} & \cellgray \good{19.49} & \cellgray \good{35.15} & \cellgray \good{21.62} & \cellgray \good{17.71} & \cellgray 30.51 & \cellgray 26.27 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance comparison between correct and original answers using PMET and our editors, with an edit batch size of 1. The type of edited fact—Pre, Mid, or Post—depends on the edited data position within the multi-hop reasoning chain. Average accuracy is calculated as the weighted average of results from these three categories, which have respective quantities of 1824, 390, and 786. Additionally,  +CoT denoted the performance incorporating a Chain-of-thought (CoT) prompt,  which can significantly enhance model performance for reasoning tasks. }
%     \label{tab:main_ablation}
% \end{table}
% \vspace{-0.05in}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \renewcommand{\arraystretch}{1.5}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{ 
\begin{tabular}{cccccccc}
\toprule
\multicolumn{3}{c}{\textbf{One-Stage Edit}}                                            & \multicolumn{3}{c}{\textbf{Two-Stage Edit}}                                 & \textbf{Multi-hop Acc} & \textbf{Efficacy} \\ \midrule
\textbf{Data}               & \textbf{Layers}          & \textbf{Position}             & \textbf{Data}               & \textbf{Layers}          & \textbf{Position}  &                             &                           \\ \midrule
\multirow{2}{*}{Single-hop} & Shallow                  & Subject Last                  & \multirow{5}{*}{×}          & \multirow{5}{*}{×}       & \multirow{5}{*}{×} & 11.70                        & 94.62                     \\ \cline{2-3}
                            & Deeper  & \rule{0pt}{2.5ex}Last                          &                             &                          &                    & 12.10                           & 97.68                          \\ \cline{1-3}
\multirow{3}{*}{Sup}        & Shallow                  & \rule{0pt}{2.5ex}Last                  &           &       &  & 10.00                        & 40.45                     \\ \cline{2-3}
                            & \multirow{2}{*}{Deeper}  & \rule{0pt}{2.5ex}Subject Last                  &                             &                          &                    & 9.03                        & 13.64                     \\
                            &                          & Last                          &                             &                          &                    & \underline{15.50}                       & 54.15                     \\ \midrule
\multirow{6}{*}{Single-hop} & \multirow{6}{*}{Shallow} & \multirow{6}{*}{Subject Last} & \multirow{2}{*}{Single-hop} & \multirow{2}{*}{Deeper}  & Subject Last       & 11.85                       & 95.21                     \\
                            &                          &                               &                             &                          & Last               & 11.33                       & 98.90                      \\ \cline{4-6}
                            &                          &                               & \multirow{4}{*}{Sup}        & \multirow{2}{*}{Shallow} & \rule{0pt}{2.5ex}Subject Last       & 13.97                       & 92.41                     \\
                            &                          &                               &                             &                          & Last               & 12.33                       & 93.45                     \\ \cline{5-6}
                            &                          &                               &                             & \multirow{2}{*}{Deeper}  &\rule{0pt}{2.5ex} Subject Last       & 12.90                        & 94.69                     \\
                            &                          &                               &                             &                          & Last               & \textbf{17.40}                        & 94.74                     \\ 
\bottomrule
\end{tabular}
}
\caption{Comparison of different methods across batch sizes, hop numbers, and edit instances.}
    \label{tab:main_ablation}
\end{table*}

==> text/results/zhexian.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/Batch_size.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/hop_zhexian.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.7\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pdf/edit-zhexian.pdf}
    \end{minipage}
    \caption{\textbf{Multi-hop Acc} Performance Comparison of different methods across batch sizes, hop numbers, and edit instances. \textbf{Base} in this table represents unmodified GPT-J-6B model, and we report its performance on \textbf{unedited answer} with CoT.}
    \label{fig:comparison_of_methods}
\end{figure}


